A Comprehensive Study of Broad Absorption Line Quasars: I. Prevalence of HeI* Absorption Line Multiplets in Low-Ionization Objects

Neutral Helium multiplets, HeI*3189,3889,10830 are very useful diagnostics to the geometry and physical conditions of the absorbing gas in quasars. So far only a handful of HeI* detections have been reported. Using a newly developed method, we detected HeI*3889 absorption line in 101 sources of a well-defined sample of 285 MgII BAL quasars selected from the SDSS DR5. This has increased the number of HeI* BAL quasars by more than one order of magnitude. We further detected HeI*3189 in 50% (52/101) quasars in the sample. The detection fraction of HeI* BALs in MgII BAL quasars is about 35% as a whole, and increases dramatically with increasing spectral signal-to-noise ratios, from 18% at S/N <= 10 to 93% at S/N >= 35. This suggests that HeI* BALs could be detected in most MgII LoBAL quasars, provided spectra S/N is high enough. Such a surprisingly high HeI* BAL fraction is actually predicted from photo-ionization calculations based on a simple BAL model. The result indicates that HeI* absorption lines can be used to search for BAL quasars at low-z, which cannot be identified by ground-based optical spectroscopic survey with commonly seen UV absorption lines. Using HeI*3889, we discovered 19 BAL quasars at z<0.3 from available SDSS spectral database. The fraction of HeI* BAL quasars is similar to that of LoBAL objects.

==> table3_complete.tex <==
\begin{landscape}

\pagestyle{empty}
\begin{deluxetable}{lrrrrrrrrrrrr}
\tablewidth{0pc}
\tablecolumns{13}
\tabletypesize{\scriptsize}
\tablecaption{The parent sample of \mgii~BAL Quasars in the SDSS DR5\label{tab:dr5mg2table}}
\tablehead{
  \colhead{SDSS Name\tablenotemark{a}}  &
  \colhead{$z$}          &  \colhead{Spectrum\tablenotemark{b}}   &
  \colhead{Mg\,II\tablenotemark{c} }       &  \colhead{Mg\,II\tablenotemark{d}}     & \colhead{Mg\,II\tablenotemark{e}}      &
  \colhead{Mg\,II\tablenotemark{f}}       & \colhead{Mg\,II\tablenotemark{g}}      & \colhead{Mg\,II\tablenotemark{h}} &
  \colhead{Mg\,II\tablenotemark{i}}       & \colhead{Ref.}        \\
  \colhead{}             &
  \colhead{}             & \colhead{}            &
  \colhead{EW (\AA)}     & \colhead{AI (km s$^{-1}$)}& \colhead{$d_{\rm abs}$} &
  \colhead{$v_{\rm max}$ (km s$^{-1}$)}  & \colhead{$v_{\rm min}$ (km s$^{-1}$)} & 
  \colhead{$v_{\rm avg}$ (km s$^{-1}$)} &
  \colhead{S/N}          & \colhead{}
}
\startdata

J000009.26+151754.5  & 1.197 &52251-0751-354 &10.15 $\pm$0.86 & 1282 & 0.80&-4104  & -126   &-1457  &9.1  &T06,Z10  \\ 
J002623.78+135523.5  & 1.319 &52233-0753-002 &24.81 $\pm$1.71 & 2547 & 0.45&-17685 & -6550  &-11943 &14.0 &T06,G09,Z10   \\ 
J004610.17+000449.7  & 0.826 &52199-0691-494 &4.92  $\pm$1.2  & 391  & 0.33&-1846  & 567    &-699   &10.3 &Z10 \\ 
J005722.48+010101.8  & 1.146 &51783-0395-417 &3.75  $\pm$0.66 & 420  & 0.40&-5249  & -3001  &-4204  &11.3 &T06,Z10  \\ 
J010352.46+003739.7  & 0.705 &51816-0396-471 &5.34  $\pm$0.44 & 556  & 0.28&-11571 & -8433  &-10071 &23.7 &T06,G09,Z10   \\ 
J011117.34+142653.6  & 1.155 &51821-0423-310 &4.51  $\pm$0.51 & 510  & 0.39&-4427  & -2652  &-3614  &20.3 &T06 \\ 
J013816.16+140431.6  & 0.877 &51882-0426-494 &6.25  $\pm$1.08 & 657  & 0.64&-5167  & -2850  &-4050  &6.6  &T06 \\ 
J013853.94-101125.7  & 1.305 &52145-0663-217 &7.86  $\pm$1.07 & 702  & 0.29&-10090 & -5311  &-7844  &16.8 &T06,G09,T06   \\ 
J014012.07+130241.8  & 1.188 &51882-0426-081 &8.30  $\pm$1.21 & 887  & 0.55&-4994  & -2196  &-3697  &5.4  &T06,G09  \\ 
J014534.36+143136.9  & 0.636 &51820-0429-372 &4.67  $\pm$0.84 & 517  & 0.50&-1888  & -29    &-1016  &10.1 &T06 \\ 
J014950.96-010314.1  & 1.082 &51793-0402-260 &4.69  $\pm$0.50 & 467  & 0.25&-9342  & -5841  &-7640  &27.3 &T06,Z10  \\ 
J015636.03+135212.3a & 1.129 &51900-0427-354 &7.70  $\pm$0.83 & 877  & 0.73&-4044  & -2267  &-3209  &10.0 &T06,Z10  \\ 
J015636.03+135212.3b & 1.129 &51900-0427-354 &5.06  $\pm$0.95 & 456  & 0.54&-6420  & -4793  &-5603  &10.0 &T06,Z10  \\ 
J020105.14+000617.9  & 1.205 &51871-0403-593 &6.47  $\pm$0.76 & 643  & 0.34&-3684  & 715    &-1827  &23.4 &T06,G09,Z10   \\ 
J023102.49-083141.2  & 0.587 &51908-0454-582 &5.36  $\pm$0.91 & 552  & 0.30&-4939  & -1660  &-3167  &12.9 &T06,G09,Z10   \\ 
J023153.64-093333.6  & 0.555 &51908-0454-017 &3.84  $\pm$0.82 & 400  & 0.43&-2064  & -136   &-1197  &6.9  &T06 \\ 
J023445.76-085908.5  & 1.275 &51909-0455-238 &10.36 $\pm$1.92 & 1072 & 0.37&-9980  & -4043  &-7174  &11.4 &T06,Z10,G09   \\ 
J024220.10-085332.7  & 0.800 &51910-0456-291 &4.58  $\pm$0.72 & 500  & 0.36&-4601  & -2211  &-3372  &11.4 &T06 \\ 
J024254.66-072205.6  & 1.217 &51910-0456-378 &15.48 $\pm$0.62 & 1615 & 0.94&-2517  & 28     &-1311  &14.0 &T06,G09,Z10   \\ 
J025026.66+000903.3  & 0.597 &51871-0409-553 &10.32 $\pm$1.56 & 946  & 0.59&-3052  & 387    &-1386  &4.9  &T06,G09,Z10   \\ 
J025204.17+010710.5  & 1.223 &51816-0410-321 &41.41 $\pm$5.46 & 2914 & 0.88&-19516 & -13049 &-16259 &3.9  &T06 \\ 
J025754.90-072449.5  & 1.023 &51901-0457-547 &5.95  $\pm$1.15 & 658  & 0.54&-3146  & -468   &-1915  &9.6  &T06,Z10  \\ 
J025813.67-011347.2  & 1.165 &52614-1068-004 &5.13  $\pm$1.32 & 449  & 0.35&-13531 & -11346 &-12448 &9.2  &G09 \\ 
J033438.28-071149.0  & 0.635 &51910-0461-074 &6.13  $\pm$0.29 & 726  & 0.45&-7821  & -5728  &-6706  &30.9 &T06 \\ 
J073122.84+430241.0  & 0.975 &53312-1865-044 &5.61  $\pm$1.22 & 432  & 0.31&-6701  & -3578  &-4881  &9.6  &Z10 \\ 
J074554.74+181817.0  & 1.054 &52939-1582-256 &12.30 $\pm$0.73 & 1329 & 0.80&-3971  & -613   &-1887  &12.0 &G09,Z10  \\ 
J075325.52+414842.9  & 1.349 &51882-0435-408 &3.36  $\pm$0.88 & 341  & 0.38&-4192  & -1867  &-3026  &15.8 &T06 \\ 
J075927.12+363431.5  & 0.983 &52238-0757-474 &15.20 $\pm$1.61 & 1606 & 0.50&-8378  & -1311  &-4118  &10.6 &T06,G09,Z10   \\ 
J080248.19+551328.8  & 0.664 &53384-1871-440 &17.03 $\pm$0.52 & 809  & 0.94&-1123  & 1434   &96     &11.7 &G09 \\ 
J080525.11+274321.8  & 0.895 &52581-0929-571 &4.75  $\pm$0.67 & 557  & 0.77&-2075  & -79    &-953   &7.9  &T06 \\ 
J080559.43+563025.8  & 0.982 &53386-1872-311 &11.53 $\pm$1.03 & 1225 & 0.57&-4931  & -1445  &-3263  &8.5  &G09,Z10  \\ 
J080934.64+254837.9  & 0.545 &52670-1205-588 &7.28  $\pm$0.70 & 402  & 0.53&-1993  & 1388   &-113   &19.1 &Z10,T06  \\ 
J080957.38+181804.4  & 0.969 &53319-1923-023 &25.61 $\pm$0.64 & 2729 & 0.97&-6028  & -701   &-2881  &23.6 &Z10 \\ 
J081312.61+432640.1  & 1.090 &52207-0547-274 &3.13  $\pm$0.87 & 364  & 0.38&-1862  & 66     &-1051  &13.9 &T06 \\ 
J081314.80+385720.4  & 0.925 &52254-0759-133 &2.92  $\pm$1.12 & 273  & 0.23&-5482  & -3440  &-4417  &9.0  &T06,Z10  \\ 
J081655.34+074311.5  & 0.645 &53083-1757-423 &3.39  $\pm$0.68 & 367  & 0.25&-5593  & -2663  &-4288  &14.0 &Z10 \\ 
J081819.29+562307.6  & 0.989 &53386-1872-105 &9.91  $\pm$0.70 & 1308 & 0.76&-5263  & -405   &-2147  &13.8 &G09,Z10  \\ 
J081820.31+200046.1  & 0.986 &53327-1925-040 &3.79  $\pm$0.72 & 406  & 0.29&-2844  & -785   &-1843  &16.4 &Z10 \\ 
J082052.63+401521.4  & 1.163 &52264-0760-085 &2.42  $\pm$0.57 & 286  & 0.24&-7145  & -4911  &-5974  &12.5 &T06 \\ 
J082231.53+231152.0  & 0.653 &53317-1926-546 &7.18  $\pm$0.77 & 681  & 0.48&-2393  & 638    &-917   &28.6 &G09,Z10  \\ 
J082525.52+352005.7  & 0.945 &52668-1197-350 &4.70  $\pm$1.03 & 480  & 0.33&-5113  & -2590  &-3829  &8.1  &T06,Z10  \\ 
J083000.35+343238.7  & 0.740 &52668-1197-098 &3.38  $\pm$0.91 & 363  & 0.28&-6756  & -4451  &-5665  &9.2  &T06 \\ 
J083522.77+424258.3  & 0.807 &52232-0762-085 &7.40  $\pm$0.48 & 627  & 0.83&-2247  & 508    &-529   &24.2 &T06 \\ 
J083525.98+435211.3  & 0.568 &52232-0762-175 &29.15 $\pm$1.07 & 2950 & 0.39&-29297 & -12066 &-19729 &24.6 &T06,G09,Z10   \\ 
J083613.23+280512.1  & 0.743 &52964-1587-350 &48.22 $\pm$2.11 & 4917 & 0.74&-18005 & -5394  &-11113 &9.1  &G09,Z10  \\ 
J084041.05+504107.7  & 1.130 &51873-0445-515 &5.42  $\pm$0.47 & 576  & 0.60&-2710  & -650   &-1757  &11.3 &G09 \\ 
J084044.41+363327.8  & 1.235 &52320-0864-149 &31.79 $\pm$0.23 & 3403 & 0.95&-5025  & -508   &-2695  &45.0 &T06,G09,Z10   \\ 
J084440.80+250253.2  & 1.001 &53347-1930-036 &8.55  $\pm$0.98 & 872  & 0.42&-8832  & -4509  &-6518  &11.3 &Z10 \\ 
J084638.50+225753.8  & 0.840 &53379-2085-315 &14.56 $\pm$1.34 & 1424 & 0.57&-8224  & -4029  &-6138  &7.0  &G09,Z10  \\ 
J084716.03+373218.0  & 0.453 &52323-0865-094 &17.85 $\pm$2.55 & 1738 & 0.36&-17133 & -9275  &-13699 &11.6 &Z10 \\ 
J084824.14+034542.3  & 0.699 &52224-0564-575 &5.26  $\pm$1.01 & 540  & 0.47&-1825  & 311    &-816   &10.9 &T06,G09  \\ 
J084953.70+021709.4  & 1.112 &52224-0564-010 &3.84  $\pm$0.98 & 313  & 0.27&-4046  & -2269  &-3149  &12.4 &T06,G09,Z10   \\ 
J085007.76+081056.4  & 1.141 &52972-1299-354 &6.70  $\pm$0.78 & 713  & 0.67&-2912  & -714   &-1849  &12.3 &G09 \\ 
J085040.44+333500.6  & 1.055 &52701-1210-175 &5.36  $\pm$2.06 & 531  & 0.35&-10058 & -6701  &-8399  &6.0  &T06 \\ 
J085053.12+445122.4  & 0.542 &52605-0897-359 &3.85  $\pm$0.53 & 432  & 0.21&-5767  & -2566  &-4032  &27.6 &T06 \\ 
J085215.65+492040.8  & 0.567 &51993-0551-274 &8.63  $\pm$0.75 & 1004 & 0.85&-2198  & -133   &-1137  &8.7  &T06,Z10  \\ 
J085357.88+463350.6  & 0.549 &52238-0764-248 &6.10  $\pm$0.58 & 658  & 0.44&-4403  & -1187  &-3055  &18.9 &T06,Z10  \\ 
J090035.42+071811.9  & 1.210 &52674-1191-329 &5.53  $\pm$1.07 & 618  & 0.48&-10459 & -7847  &-9247  &8.3  &T06,G09  \\ 
J090056.89+021702.6  & 0.830 &51913-0469-575 &8.46  $\pm$1.04 & 784  & 0.66&-2595  & 710    &-685   &7.8  &T06 \\ 
J090132.62+233257.7  & 0.845 &53401-2086-209 &10.26 $\pm$1.18 & 667  & 0.40&-5568  & -2090  &-3711  &10.5 &Z10 \\ 
J090154.96+380534.4  & 1.038 &52705-0936-498 &11.55 $\pm$0.95 & 1116 & 0.32&-11771 & -5464  &-8376  &19.6 &T06,Z10  \\ 
J090321.30+244928.0  & 1.235 &53401-2086-466 &28.53 $\pm$5.05 & 2040 & 0.85&-23611 & -17954 &-20731 &4.4  &G09 \\ 
J090825.06+014227.7  & 1.002 &51924-0471-499 &8.94  $\pm$0.91 & 886  & 0.32&-12119 & -7104  &-9727  &16.2 &T06,G09,Z10   \\ 
J091146.06+403501.0  & 0.441 &52668-1200-015 &27.31 $\pm$2.16 & 2915 & 0.67&-9793  & -1663  &-5529  &5.3  &Z10 \\ 
J091214.02+424740.5  & 1.327 &52674-1201-384 &9.28  $\pm$1.78 & 566  & 0.35&-11721 & -8450  &-10223 &11.8 &T06,G09,Z10   \\ 
J091854.48+583339.6  & 1.315 &51907-0484-598 &10.35 $\pm$0.99 & 575  & 0.87&-1316  & 1101   &-4     &8.8  &T06 \\ 
J092035.59+524006.2  & 0.793 &51999-0553-612 &4.43  $\pm$1.38 & 365  & 0.63&-1170  & 555    &-405   &8.6  &T06 \\ 
J092157.62+103539.0  & 0.548 &53050-1740-170 &19.19 $\pm$1.54 & 2068 & 0.55&-10212 & -2983  &-6137  &7.7  &G09,Z10  \\ 
J092441.08-001729.6  & 0.707 &52000-0474-167 &2.14  $\pm$0.55 & 235  & 0.25&-3094  & -898   &-2049  &18.7 &T06 \\ 
J092515.40+493539.8  & 1.294 &52637-0900-447 &3.78  $\pm$1.06 & 250  & 0.23&-7725  & -5563  &-6566  &14.9 &T06,G09  \\ 
J092928.63+324129.8  & 0.776 &53386-1941-404 &4.48  $\pm$0.70 & 503  & 0.20&-10335 & -5425  &-8154  &17.6 &Z10 \\ 
J093034.79+570520.6  & 0.637 &51911-0452-210 &3.57  $\pm$0.63 & 391  & 0.23&-10718 & -7705  &-9022  &12.6 &T06,Z10  \\ 
J093228.56+555344.8  & 0.878 &51991-0556-251 &15.24 $\pm$0.81 & 1659 & 0.65&-8975  & -3359  &-5663  &12.4 &T06,G09,Z10   \\ 
J093759.60+453801.8  & 0.429 &52672-1202-330 &4.21  $\pm$0.96 & 464  & 0.39&-2297  & 527    &-837   &12.3 &Z10 \\ 
J093919.87+440449.5  & 1.307 &52672-1202-124 &2.28  $\pm$0.75 & 217  & 0.25&-8519  & -6701  &-7701  &16.2 &T06 \\ 
J093953.44+033229.7  & 0.927 &52266-0570-310 &4.51  $\pm$0.76 & 376  & 0.31&-6438  & -4607  &-5611  &8.1  &T06 \\ 
J094225.42+565613.0  & 0.833 &52253-0557-359 &26.85 $\pm$1.87 & 2446 & 0.37&-19779 & -8861  &-14480 &14.1 &T06 \\ 
J094355.00+560649.0a & 1.055 &52253-0557-299 &10.75 $\pm$0.71 & 980  & 0.89&-2059  & 352    &-743   &8.3  &T06,G09,T06   \\ 
J094355.00+560649.0b & 1.055 &52253-0557-299 &3.71  $\pm$1.01 & 366  & 0.45&-4994  & -3223  &-4117  &8.3  &T06,G09,T06   \\ 
J094443.13+062507.4  & 0.695 &52710-0993-535 &14.73 $\pm$0.98 & 1575 & 0.48&-9285  & -2650  &-6739  &40.8 &T06,G09,Z10   \\ 
J094759.66+120537.7  & 1.287 &53053-1742-624 &5.99  $\pm$0.79 & 626  & 0.50&-4260  & -1730  &-2877  &13.0 &Z10,G09  \\ 
J094939.93+393642.9  & 0.654 &52765-1277-337 &36.17 $\pm$2.99 & 3743 & 0.71&-12346 & -3469  &-7424  &4.1  &T06,G09  \\ 
J095057.56+542919.4  & 1.194 &52282-0769-507 &14.36 $\pm$1.41 & 1442 & 0.68&-5631  & -1536  &-3588  &7.1  &T06,G09  \\ 
J095914.91+131639.5  & 1.009 &53055-1744-362 &13.84 $\pm$1.38 & 1489 & 0.43&-8847  & -3092  &-5887  &7.6  &G09,Z10  \\ 
J100552.24+025902.4  & 0.908 &52235-0501-562 &3.28  $\pm$0.49 & 343  & 0.33&-3666  & -1818  &-2699  &18.6 &T06 \\ 
J101139.21+415639.7  & 1.201 &53034-1357-324 &14.44 $\pm$3.15 & 1301 & 0.81&-17143 & -13274 &-15144 &5.2  &G09 \\ 
J101151.95+542942.6  & 0.536 &52652-0945-028 &5.01  $\pm$1.33 & 532  & 0.46&-2563  & -363   &-1620  &5.7  &T06 \\ 
J101203.31+492148.2a & 0.739 &52706-1007-127 &5.38  $\pm$0.60 & 585  & 0.48&-2721  & -178   &-1294  &14.8 &T06,G09,Z10   \\ 
J101203.31+492148.2b & 0.739 &52706-1007-127 &7.58  $\pm$0.98 & 712  & 0.32&-7946  & -3542  &-5816  &14.8 &T06,G09,Z10   \\ 
J101302.06+361510.7  & 0.836 &53357-1954-406 &11.71 $\pm$1.46 & 1468 & 0.46&-11686 & -3882  &-7610  &9.2  &Z10 \\ 
J102021.21+121909.1  & 0.480 &53062-1746-215 &38.08 $\pm$4.47 & 3894 & 0.74&-20399 & -8030  &-13827 &6.2  &G09,Z10  \\ 
J102036.10+602339.0  & 0.994 &52370-0771-011 &26.59 $\pm$1.29 & 1883 & 0.97&-3218  & 1744   &-619   &6.8  &T06,G09,Z10   \\ 
J102225.67+602630.2  & 1.173 &52316-0559-447 &5.61  $\pm$0.98 & 571  & 0.28&-7780  & -4600  &-6045  &10.9 &T06,Z10  \\ 
J102249.27+130125.0  & 1.217 &53062-1746-151 &22.52 $\pm$1.10 & 2378 & 0.88&-6345  & -2260  &-4133  &7.2  &G09 \\ 
J102802.33+592906.7  & 0.536 &52316-0559-582 &10.13 $\pm$0.83 & 1063 & 0.71&-2557  & 126    &-1163  &9.1  &T06,G09,Z10   \\ 
J102839.11+450009.4  & 0.585 &52990-1429-401 &6.73  $\pm$0.68 & 693  & 0.45&-2324  & 85     &-1069  &32.7 &G09,Z10  \\ 
J102943.75+370127.2  & 1.344 &53415-1957-601 &7.05  $\pm$1.05 & 678  & 0.80&-1512  & 211    &-611   &6.0  &G09 \\ 
J103036.93+312028.8  & 0.876 &53440-1959-121 &10.95 $\pm$0.39 & 1165 & 0.69&-6485  & -3564  &-5084  &22.1 &G09,Z10  \\ 
J103110.64+395322.3  & 1.081 &52998-1428-608 &4.99  $\pm$0.52 & 552  & 0.48&-5516  & -2654  &-4009  &17.3 &Z10 \\ 
J103113.38+344613.5  & 0.942 &53385-1958-635 &6.99  $\pm$0.71 & 736  & 0.54&-2961  & -281   &-1514  &13.1 &G09 \\ 
J103255.37+083503.2  & 0.894 &52734-1240-316 &9.52  $\pm$0.66 & 1021 & 0.53&-4657  & -962   &-2918  &21.0 &T06,G09,Z10   \\ 
J103621.60+393701.6  & 0.802 &53002-1430-555 &8.91  $\pm$0.96 & 921  & 0.55&-3686  & 228    &-1537  &31.7 &G09,Z10  \\ 
J103739.61+501505.7  & 0.947 &52354-0875-511 &5.31  $\pm$0.98 & 587  & 0.32&-3996  & -224   &-2147  &8.7  &T06 \\ 
J103824.47-010538.9  & 0.773 &51913-0274-205 &10.46 $\pm$1.25 & 445  & 0.85&-1331  & 1294   &107    &5.8  &T06 \\ 
J103929.00+472436.9  & 1.110 &52620-0962-492 &16.78 $\pm$2.29 & 1714 & 0.37&-18147 & -9984  &-13720 &8.6  &T06,G09,Z10   \\ 
J103933.38+035200.4  & 0.916 &52339-0578-294 &5.55  $\pm$1.25 & 587  & 0.43&-5894  & -3241  &-4620  &6.1  &T06 \\ 
J104035.07+623329.5  & 1.174 &52376-0773-181 &3.09  $\pm$0.94 & 345  & 0.31&-6852  & -4480  &-5588  &9.3  &G09 \\ 
J104116.79+035511.4  & 1.246 &52367-0577-017 &3.25  $\pm$1.01 & 359  & 0.33&-4852  & -2806  &-3871  &5.2  &T06,Z10  \\ 
J104132.96+513657.0  & 0.735 &52649-1010-294 &5.20  $\pm$0.69 & 499  & 0.17&-10098 & -4844  &-7539  &19.8 &T06 \\ 
J104210.43+501609.1  & 0.789 &52354-0875-583 &11.94 $\pm$0.53 & 1287 & 0.86&-3612  & -732   &-2383  &18.1 &T06,G09,Z10   \\ 
J104459.60+365605.1a & 0.701 &53463-2090-329 &10.44 $\pm$0.29 & 1113 & 0.82&-2123  & 80     &-1129  &29.2 &G09,Z10  \\ 
J104459.60+365605.1b & 0.701 &53463-2090-329 &17.76 $\pm$0.22 & 1786 & 1.00&-5736  & -3013  &-4283  &29.2 &G09,Z10  \\ 
J104459.60+365605.1c & 0.701 &53463-2090-329 &11.34 $\pm$0.61 & 1057 & 0.24&-18137 & -10574 &-14369 &29.2 &G09,Z10  \\ 
J104705.08+590728.4  & 0.392 &52427-0949-326 &6.18  $\pm$1.62 & 501  & 0.51&-1688  & 726    &-527   &6.4  &G09 \\ 
J104838.65+603933.1  & 1.274 &52295-0561-514 &3.84  $\pm$0.95 & 406  & 0.30&-9085  & -6731  &-7813  &9.9  &T06,Z10  \\ 
J104845.83+353110.7  & 1.011 &53463-2090-131 &4.52  $\pm$0.41 & 500  & 0.45&-4285  & -2235  &-3230  &20.6 &Z10 \\ 
J105102.78+525049.8  & 0.543 &52649-1010-556 &4.06  $\pm$1.57 & 511  & 0.46&-2497  & -159   &-1326  &9.3  &T06,G09  \\ 
J105259.99+065358.0  & 0.724 &52670-1001-080 &33.96 $\pm$1.62 & 3583 & 0.52&-17034 & -3903  &-9687  &11.9 &T06,G09,Z10   \\ 
J105404.72+042939.3  & 0.579 &52338-0579-072 &2.86  $\pm$1.11 & 326  & 0.39&-2013  & -293   &-1159  &4.6  &T06 \\ 
J105638.08+494943.3  & 1.148 &52669-0876-110 &1.75  $\pm$0.28 & 171  & 0.14&-12043 & -10180 &-11179 &35.5 &T06 \\ 
J105748.63+610910.8  & 1.274 &52286-0774-278 &7.88  $\pm$1.37 & 801  & 0.89&-10103 & -7959  &-9245  &8.2  &T06 \\ 
J105823.13+600805.6  & 1.071 &52286-0774-289 &4.29  $\pm$0.6  & 444  & 0.27&-10800 & -7923  &-9480  &15.3 &T06,Z10  \\ 
J110108.43+515021.9  & 0.968 &52353-0877-402 &4.91  $\pm$0.49 & 581  & 0.24&-11676 & -6856  &-9251  &23.0 &T06,Z10  \\ 
J110440.82-000441.6  & 1.344 &51908-0277-077 &9.54  $\pm$1.13 & 1035 & 0.57&-6164  & -1252  &-3276  &12.6 &T06,Z10,G09   \\ 
J110810.99+352927.4  & 1.062 &53466-2034-513 &4.96  $\pm$0.95 & 530  & 0.36&-4893  & -2162  &-3556  &8.2  &Z10 \\ 
J110839.62+532721.4  & 0.878 &52652-1011-035 &18.55 $\pm$1.44 & 1342 & 0.95&-2750  & 899    &-632   &4.4  &T06,G09  \\ 
J111013.79+523607.2  & 1.009 &52649-1012-259 &3.01  $\pm$0.55 & 232  & 0.14&-10726 & -8453  &-9560  &26.9 &T06,Z10  \\ 
J111040.48+433821.3  & 1.230 &53061-1364-154 &6.32  $\pm$1.04 & 677  & 0.34&-4975  & -1559  &-3316  &10.7 &G09,Z10  \\ 
J111628.00+434505.8  & 0.801 &53061-1364-095 &6.73  $\pm$0.52 & 710  & 0.33&-6364  & -2416  &-4166  &22.6 &Z10 \\ 
J112349.16+135220.6  & 0.928 &53383-1753-093 &26.66 $\pm$2.19 & 2765 & 0.44&-14895 & -3582  &-8448  &10.7 &G09,Z10  \\ 
J112632.81+430938.5  & 0.436 &53062-1365-036 &9.50  $\pm$0.86 & 939  & 0.84&-2374  & 311    &-853   &8.5  &Z10 \\ 
J112730.71+423039.0  & 0.531 &53055-1443-374 &16.87 $\pm$3.00 & 1015 & 0.29&-22313 & -16237 &-19031 &10.0 &G09,Z10  \\ 
J112822.42+482310.1  & 0.541 &52642-0966-203 &13.33 $\pm$0.90 & 1306 & 0.36&-5868  & 913    &-2228  &18.5 &T06,Z10  \\ 
J112828.31+011337.9  & 0.893 &51992-0512-123 &14.33 $\pm$0.75 & 1011 & 0.84&-2304  & 1838   &-338   &11.2 &T06,G09,Z10   \\ 
J112901.71+050617.0  & 1.282 &52642-0837-400 &13.84 $\pm$1.50 & 1477 & 0.91&-5547  & -1795  &-3885  &6.6  &T06,G09  \\ 
J112912.27+422853.9  & 0.582 &53055-1443-415 &4.18  $\pm$0.67 & 411  & 0.27&-6995  & -4148  &-5438  &10.6 &Z10 \\ 
J113349.81+361027.3  & 1.158 &53468-2113-608 &17.1  $\pm$1.67 & 1767 & 0.56&-8960  & -3549  &-6377  &8.3  &G09 \\ 
J113355.22+111208.8  & 0.763 &53083-1607-298 &14.95 $\pm$1.56 & 1441 & 0.35&-13062 & -4207  &-8465  &12.8 &Z10 \\ 
J113704.85+055240.4  & 0.915 &52378-0838-328 &5.24  $\pm$0.96 & 581  & 0.41&-6614  & -2738  &-4363  &10.6 &T06 \\ 
J113807.83+531231.6a & 0.790 &52367-0880-404 &2.11  $\pm$0.44 & 222  & 0.26&-2084  & -571   &-1445  &12.0 &T06,Z10  \\ 
J113807.83+531231.6b & 0.790 &52367-0880-404 &8.50  $\pm$0.51 & 916  & 0.66&-4543  & -2221  &-3391  &12.0 &T06,Z10  \\ 
J113940.42+451207.0  & 1.141 &53083-1367-454 &22.39 $\pm$1.18 & 2306 & 0.55&-13199 & -3735  &-7642  &16.7 &G09,Z10  \\ 
J114033.47+150701.7  & 1.250 &53386-1755-589 &7.41  $\pm$0.92 & 790  & 0.48&-4960  & -1544  &-3118  &12.5 &G09,Z10  \\ 
J114043.62+532438.9  & 0.530 &52734-1015-085 &9.51  $\pm$0.64 & 1031 & 0.68&-3557  & -745   &-2236  &8.7  &T06,G09,Z10   \\ 
J114111.61-014306.6  & 1.266 &52282-0328-417 &3.88  $\pm$0.69 & 463  & 0.29&-4552  & -1406  &-2911  &36.1 &T06,G09  \\ 
J114209.01+070957.7  & 0.497 &53383-1621-306 &16.62 $\pm$2.23 & 1392 & 0.39&-19365 & -12564 &-16162 &13.3 &G09 \\ 
J114516.73+493259.4  & 1.158 &52636-0967-558 &9.20  $\pm$1.13 & 954  & 0.44&-8245  & -3163  &-5528  &16.4 &T06,G09  \\ 
J114600.32+504734.0a & 1.081 &52636-0967-562 &6.64  $\pm$0.80 & 604  & 0.31&-5564  & -2360  &-3988  &19.1 &T06,G09,Z10   \\ 
J114600.32+504734.0b & 1.081 &52636-0967-562 &5.68  $\pm$0.66 & 574  & 0.34&-9737  & -6849  &-8234  &19.1 &T06,G09,Z10   \\ 
J114740.33+373438.9  & 1.297 &53442-1997-143 &33.23 $\pm$2.57 & 3398 & 0.55&-17699 & -6159  &-12531 &9.0  &G09 \\ 
J114754.36+040638.4  & 1.174 &52373-0839-096 &2.75  $\pm$0.91 & 287  & 0.23&-7372  & -5208  &-6252  &9.5  &T06 \\ 
J114915.30+393325.4  & 0.630 &53386-1970-137 &21.49 $\pm$1.85 & 1764 & 0.63&-6076  & -1369  &-3500  &6.6  &G09,Z10  \\ 
J115010.81+480844.3  & 1.190 &53080-1446-333 &7.05  $\pm$1.28 & 509  & 0.29&-6945  & -3825  &-5365  &10.9 &Z10 \\ 
J115511.93+465903.7  & 1.298 &53080-1446-161 &6.13  $\pm$0.63 & 643  & 0.44&-5939  & -3286  &-4726  &15.6 &G09,Z10  \\ 
J115553.87+012427.6  & 1.010 &52051-0515-043 &16.17 $\pm$0.48 & 1838 & 0.83&-5852  & -2172  &-4017  &15.8 &T06,G09,Z10   \\ 
J115816.72+132624.1  & 0.440 &53144-1610-562 &12.59 $\pm$0.67 & 1277 & 0.42&-9328  & -3924  &-6266  &24.6 &G09,Z10  \\ 
J115832.28+044208.3  & 0.896 &52375-0841-193 &4.63  $\pm$0.63 & 490  & 0.24&-7828  & -4105  &-5932  &17.0 &T06,Z10  \\ 
J115852.87-004301.9  & 0.983 &51930-0285-189 &15.83 $\pm$0.62 & 961  & 0.97&-1253  & 1233   &-113   &7.5  &T06 \\ 
J115923.83+415246.7  & 1.200 &53120-1447-068 &3.88  $\pm$0.35 & 400  & 0.28&-9303  & -6951  &-8034  &22.6 &Z10,G09  \\ 
J120049.55+632211.8  & 0.887 &52337-0778-377 &9.85  $\pm$0.53 & 1024 & 0.89&-1804  & 332    &-823   &8.8  &T06,G09  \\ 
J120146.46+630034.4  & 0.659 &52337-0778-439 &7.06  $\pm$1.87 & 618  & 0.47&-2876  & 1258   &-812   &8.2  &T06 \\ 
J120337.91+153006.6  & 1.218 &53467-1764-412 &32.85 $\pm$2.42 & 3307 & 0.45&-21653 & -7527  &-14109 &24.0 &G09,Z10  \\ 
J120813.42+023015.1  & 1.182 &52024-0517-509 &2.84  $\pm$0.49 & 279  & 0.16&-17791 & -14983 &-16373 &58.9 &T06 \\ 
J120924.07+103612.0  & 0.395 &52723-1229-489 &5.41  $\pm$0.51 & 557  & 0.38&-2199  & 280    &-940   &34.9 &G09 \\ 
J120928.11+003511.6  & 0.610 &51999-0286-594 &9.65  $\pm$3.23 & 940  & 0.77&-3560  & -886   &-2576  &1.4  &T06 \\ 
J121113.38+121937.3  & 0.465 &53149-1612-179 &12.27 $\pm$1.15 & 1341 & 0.80&-3864  & -504   &-1975  &9.6  &G09,Z10  \\ 
J121303.40-014450.9  & 0.613 &52367-0332-579 &7.70  $\pm$0.68 & 709  & 0.68&-4088  & -2037  &-3028  &12.3 &Z10,T06  \\ 
J121441.42-000137.8  & 1.046 &52023-0287-514 &36.34 $\pm$2.30 & 3705 & 0.54&-18003 & -6272  &-12449 &8.6  &T06,G09,Z10,T06    \\ 
J121806.00+101920.6  & 1.089 &52672-1230-483 &8.91  $\pm$1.42 & 899  & 0.81&-2097  & 314    &-833   &4.9  &T06 \\ 
J121907.80-005609.2  & 0.638 &52000-0288-132 &13.64 $\pm$1.49 & 1320 & 0.88&-3210  & -808   &-1975  &3.6  &T06,G09  \\ 
J122020.29+575637.6  & 1.307 &52791-1315-498 &13.92 $\pm$2.22 & 1330 & 0.82&-8465  & -4749  &-6722  &5.1  &T06 \\ 
J122043.21-013215.3  & 0.448 &52313-0333-540 &7.31  $\pm$0.93 & 712  & 0.68&-1648  & 213    &-698   &4.9  &Z10 \\ 
J122305.79+085651.4  & 1.091 &52725-1231-246 &2.95  $\pm$0.80 & 316  & 0.32&-2896  & -974   &-2136  &11.2 &T06 \\ 
J122424.17+593528.5  & 0.899 &52409-0955-033 &3.46  $\pm$1.19 & 381  & 0.35&-4626  & -2030  &-3432  &8.4  &T06 \\ 
J122614.97+120925.4  & 0.871 &53120-1614-145 &7.38  $\pm$0.80 & 796  & 0.58&-2693  & -287   &-1353  &15.8 &Z10 \\ 
J122703.19+505356.2  & 0.765 &52644-0971-459 &5.96  $\pm$0.73 & 663  & 0.66&-2134  & -138   &-1114  &8.4  &T06 \\ 
J122847.60+490431.8  & 0.954 &52644-0971-094 &8.04  $\pm$1.23 & 869  & 0.28&-9791  & -4872  &-7124  &8.5  &T06,G09,Z10   \\ 
J123218.09+410637.9  & 1.326 &53433-1984-363 &14.37 $\pm$1.09 & 1454 & 0.70&-3753  & 506    &-1419  &11.8 &G09,Z10  \\ 
J124300.87+153510.6  & 0.562 &53502-1769-584 &12.83 $\pm$0.66 & 1153 & 0.84&-2117  & 986    &-657   &13.5 &G09,Z10  \\ 
J125057.57+402100.2  & 0.607 &53431-1985-596 &19.46 $\pm$1.73 & 2089 & 0.91&-8024  & -1498  &-4017  &7.3  &Z10 \\ 
J125507.12+634423.8  & 1.067 &52316-0601-043 &27.65 $\pm$1.99 & 2822 & 0.54&-22653 & -11582 &-16543 &9.4  &T06,G09,Z10   \\ 
J130006.47+653201.7  & 1.192 &52072-0602-321 &8.06  $\pm$1.50 & 780  & 0.48&-10736 & -6172  &-8484  &9.8  &T06 \\ 
J130444.12+052820.8  & 0.935 &52439-0849-582 &6.26  $\pm$0.78 & 626  & 0.78&-2906  & -640   &-2002  &7.2  &G09 \\ 
J130741.12+503106.4  & 0.695 &52753-1281-361 &20.61 $\pm$0.86 & 2171 & 0.82&-5901  & -157   &-2884  &13.2 &T06,G09,Z10   \\ 
J130952.89+011950.6  & 0.547 &52295-0525-250 &5.08  $\pm$1.12 & 397  & 0.44&-1833  & 718    &-416   &26.9 &T06 \\ 
J131323.25+151309.6a & 1.262 &53089-1772-627 &3.50  $\pm$0.37 & 342  & 0.28&-5046  & -3070  &-4171  &26.6 &Z10,G09  \\ 
J131323.25+151309.6b & 1.262 &53089-1772-627 &7.64  $\pm$0.69 & 784  & 0.31&-11096 & -5792  &-8264  &26.6 &Z10,G09  \\ 
J131433.19+471457.7  & 0.873 &53062-1461-431 &4.94  $\pm$1.09 & 527  & 0.42&-3509  & -1041  &-2461  &9.4  &G09 \\ 
J131637.26-003636.0  & 0.930 &51985-0295-080 &16.57 $\pm$1.46 & 896  & 0.44&-3854  & 4303   &101    &20.3 &T06,G09,Z10   \\ 
J131703.87+614228.5  & 1.344 &52325-0783-040 &4.22  $\pm$1.42 & 369  & 0.39&-7271  & -5445  &-6497  &8.7  &T06 \\ 
J131823.73+123812.5  & 0.589 &53142-1697-600 &16.12 $\pm$0.94 & 1688 & 0.88&-4558  & -1274  &-2817  &8.8  &G09,Z10  \\ 
J132114.42+020225.0  & 0.582 &52312-0526-157 &5.48  $\pm$0.96 & 624  & 0.43&-5413  & -2413  &-3844  &8.9  &T06,G09,Z10,T06    \\ 
J132401.53+032020.6  & 0.926 &52312-0526-609 &13.67 $\pm$1.22 & 1298 & 0.84&-3398  & 521    &-1146  &7.9  &G09,T06  \\ 
J132439.32+421604.7  & 1.020 &53112-1462-524 &10.32 $\pm$0.93 & 1100 & 0.90&-3372  & -765   &-1937  &7.7  &G09,Z10  \\ 
J133014.48+413244.9  & 1.146 &53091-1464-339 &4.23  $\pm$0.60 & 490  & 0.42&-6689  & -3976  &-5388  &16.6 &Z10 \\ 
J133603.65+511733.6  & 1.327 &53433-1669-339 &5.43  $\pm$0.96 & 569  & 0.51&-7002  & -5107  &-6072  &11.4 &Z10 \\ 
J133833.82+034522.2  & 1.301 &52374-0853-048 &15.66 $\pm$0.97 & 967  & 0.94&-1567  & 917    &-211   &9.2  &T06,T06  \\ 
J133936.69+111949.2  & 0.650 &53502-1700-101 &4.15  $\pm$0.60 & 550  & 0.39&-6888  & -3766  &-5571  &9.3  &Z10 \\ 
J134127.40+002050.5  & 0.722 &51671-0299-464 &3.56  $\pm$0.99 & 298  & 0.28&-2847  & -1063  &-2016  &12.3 &T06 \\ 
J134410.43+535352.8  & 0.827 &52725-1042-549 &6.34  $\pm$0.99 & 598  & 0.30&-7362  & -4042  &-5789  &12.8 &T06,G09,Z10   \\ 
J134415.75+331719.1  & 0.687 &53503-2024-346 &7.04  $\pm$0.97 & 768  & 0.61&-2284  & 263    &-813   &10.4 &Z10 \\ 
J134450.16-015843.0  & 0.958 &52433-0913-381 &14.88 $\pm$1.35 & 1549 & 0.51&-11459 & -5146  &-8064  &9.2  &T06,G09,Z10   \\ 
J134830.78-015357.8  & 0.816 &52721-0914-353 &21.47 $\pm$1.62 & 2300 & 0.56&-13613 & -6739  &-9833  &7.0  &T06,G09  \\ 
J134938.48+475530.1  & 1.104 &52736-1284-551 &11.22 $\pm$1.06 & 1121 & 0.31&-13063 & -5363  &-8769  &19.6 &T06,Z10,G09   \\ 
J134951.56+040407.2  & 1.032 &52375-0855-229 &3.13  $\pm$0.79 & 323  & 0.24&-6341  & -3146  &-4891  &17.4 &T06 \\ 
J135226.34+024549.4  & 1.222 &52026-0530-588 &3.0   $\pm$0.80 & 325  & 0.22&-4525  & -2408  &-3405  &13.4 &G09,Z10  \\ 
J135418.26+585935.9  & 0.791 &52668-1158-521 &8.51  $\pm$1.11 & 871  & 0.64&-3626  & -1228  &-2534  &7.8  &T06,G09  \\ 
J135546.11+431819.8  & 1.318 &52822-1346-378 &9.55  $\pm$1.18 & 814  & 0.40&-10091 & -5990  &-8085  &12.7 &T06,G09,Z10   \\ 
J135750.89+632446.2  & 1.347 &52353-0605-392 &9.78  $\pm$1.04 & 1007 & 0.31&-8089  & -1702  &-4499  &14.4 &T06,G09  \\ 
J140025.53-012957.0a & 0.584 &52443-0915-380 &6.80  $\pm$0.79 & 442  & 0.49&-1649  & 1666   &-259   &10.8 &T06,G09,Z10   \\ 
J140025.53-012957.0b & 0.584 &52443-0915-380 &27.16 $\pm$1.66 & 2801 & 0.60&-25636 & -15798 &-20042 &10.8 &T06,G09,Z10   \\ 
J140115.74+621857.1a & 0.645 &52353-0605-147 &10.88 $\pm$1.53 & 671  & 0.86&-4006  & -2366  &-3198  &4.8  &T06 \\ 
J140115.74+621857.1b & 0.645 &52353-0605-147 &9.15  $\pm$1.27 & 747  & 0.73&-7865  & -6111  &-7095  &4.8  &T06 \\ 
J140332.86+133218.7  & 1.093 &53178-1704-195 &9.24  $\pm$0.49 & 972  & 0.89&-3350  & -881   &-1896  &15.7 &G09,Z10  \\ 
J141513.20+634037.2  & 1.334 &51988-0499-306 &3.85  $\pm$1.14 & 352  & 0.32&-5785  & -3404  &-4774  &16.9 &T06 \\ 
J141555.07+582632.8  & 1.261 &52338-0788-054 &4.96  $\pm$0.82 & 477  & 0.41&-2776  & -647   &-1872  &11.8 &T06,G09  \\ 
J142010.28+604722.3  & 1.345 &52365-0606-110 &17.82 $\pm$1.62 & 1805 & 0.88&-3571  & -622   &-2148  &9.2  &G09 \\ 
J142110.71+035439.8  & 0.831 &52049-0584-190 &6.73  $\pm$1.26 & 658  & 0.56&-3671  & -1616  &-2751  &5.2  &T06,G09  \\ 
J142116.23+052252.3  & 0.926 &52049-0584-404 &8.29  $\pm$0.63 & 875  & 0.72&-5719  & -3679  &-4793  &8.2  &T06 \\ 
J142647.47+401250.8  & 0.749 &52797-1349-348 &4.66  $\pm$0.95 & 429  & 0.58&-3460  & -1749  &-2734  &9.0  &G09 \\ 
J142649.24+032517.7  & 0.529 &52049-0584-004 &4.68  $\pm$0.60 & 549  & 0.39&-3258  & -995   &-2197  &9.4  &T06,Z10  \\ 
J142927.28+523849.5  & 0.595 &52781-1327-343 &14.32 $\pm$0.87 & 1528 & 0.44&-7761  & -1091  &-3911  &20.9 &T06,G09,Z10   \\ 
J143144.91+391910.2  & 1.091 &52797-1349-257 &4.77  $\pm$0.92 & 345  & 0.43&-1524  & 476    &-537   &16.2 &T06 \\ 
J143303.27+403105.1  & 0.446 &52797-1349-484 &5.35  $\pm$0.93 & 580  & 0.52&-3447  & -910   &-2242  &7.7  &Z10 \\ 
J143826.73+642859.8  & 1.222 &51988-0499-623 &9.92  $\pm$0.95 & 1039 & 0.32&-10271 & -3591  &-6706  &24.4 &T06,Z10,G09   \\ 
J143828.63+452108.6  & 0.427 &52731-1288-628 &6.73  $\pm$2.57 & 743  & 0.27&-10313 & -4995  &-7472  &12.7 &G09,Z10  \\ 
J144222.02+524143.2  & 1.037 &52781-1327-550 &7.69  $\pm$1.23 & 646  & 0.53&-4354  & -1618  &-2826  &8.3  &T06,G09,Z10   \\ 
J144317.71-020933.0a & 1.045 &52411-0920-232 &4.19  $\pm$0.70 & 462  & 0.44&-4219  & -2169  &-3123  &9.6  &T06,Z10  \\ 
J144317.71-020933.0b & 1.045 &52411-0920-232 &1.95  $\pm$1.00 & 189  & 0.25&-13008 & -11550 &-12311 &9.6  &T06,Z10  \\ 
J144342.21-025430.6  & 0.777 &52411-0920-258 &8.76  $\pm$0.73 & 954  & 0.98&-3145  & -1500  &-2336  &7.6  &T06 \\ 
J144436.58+425508.6  & 1.101 &52734-1289-087 &6.44  $\pm$0.72 & 688  & 0.34&-7807  & -4288  &-5931  &13.8 &T06,G09,Z10   \\ 
J144627.41+353453.5  & 0.922 &53116-1383-188 &6.86  $\pm$0.54 & 740  & 0.45&-3032  & -560   &-1833  &20.1 &G09,Z10  \\ 
J144642.26+454630.9  & 0.738 &53466-1675-168 &14.43 $\pm$1.52 & 1520 & 0.43&-9722  & -1933  &-5360  &10.3 &G09,Z10  \\ 
J144759.19+350833.5  & 0.953 &53116-1383-260 &6.56  $\pm$0.89 & 723  & 0.34&-5817  & -1999  &-4106  &13.7 &Z10 \\ 
J144903.18+503018.1  & 0.609 &52786-1328-215 &6.05  $\pm$1.12 & 871  & 0.37&-6047  & -927   &-3102  &7.8  &T06,Z10  \\ 
J145333.01+002943.6  & 1.291 &51994-0309-433 &6.70  $\pm$1.45 & 654  & 0.62&-1644  & 701    &-727   &7.2  &T06 \\ 
J145503.95+515539.8  & 1.277 &52786-1328-615 &7.23  $\pm$0.86 & 773  & 0.78&-2917  & -1134  &-1951  &8.0  &T06 \\ 
J145549.84-013018.3  & 1.321 &52380-0921-490 &4.65  $\pm$0.88 & 495  & 0.45&-5799  & -3691  &-4750  &9.5  &T06 \\ 
J145724.00+452157.8  & 0.718 &53147-1676-449 &21.59 $\pm$1.41 & 2257 & 0.41&-14325 & -5034  &-9780  &15.2 &G09,Z10  \\ 
J145736.70+523454.6  & 0.638 &52674-1164-184 &20.59 $\pm$1.09 & 2131 & 0.39&-12151 & -2104  &-6325  &16.4 &T06,G09,Z10   \\ 
J145836.73+433015.5  & 0.760 &52734-1290-601 &8.45  $\pm$1.10 & 895  & 0.36&-6969  & -2345  &-4606  &9.1  &T06,G09,Z10   \\ 
J150525.51-023853.8a & 1.159 &52426-0922-084 &3.57  $\pm$0.80 & 266  & 0.27&-4762  & -2921  &-3916  &9.2  &T06,Z10  \\ 
J150525.51-023853.8b & 1.159 &52426-0922-084 &7.32  $\pm$0.94 & 756  & 0.45&-8679  & -5577  &-6911  &9.2  &T06,Z10  \\ 
J150847.41+340437.7  & 0.788 &53108-1385-173 &7.31  $\pm$0.41 & 762  & 0.51&-2676  & 213    &-1289  &26.7 &G09,Z10  \\ 
J151053.63+574055.1  & 1.037 &52079-0612-424 &17.86 $\pm$0.75 & 1925 & 0.40&-11460 & -2350  &-6208  &18.0 &T06,G09,Z10,T06    \\ 
J151225.67+585752.2  & 0.791 &52345-0613-298 &13.64 $\pm$2.00 & 610  & 0.92&-1242  & 1245   &72     &4.4  &T06,G09  \\ 
J151545.34+031745.0  & 0.780 &52022-0591-250 &8.01  $\pm$1.18 & 893  & 0.79&-3421  & -1503  &-2416  &4.8  &T06 \\ 
J151548.67+430420.5  & 0.527 &53148-1677-027 &5.62  $\pm$1.05 & 594  & 0.52&-3528  & -1198  &-2213  &6.1  &Z10 \\ 
J152200.76+035017.0  & 0.838 &52022-0591-617 &7.51  $\pm$1.10 & 667  & 0.58&-2261  & 287    &-981   &9.5  &Z10 \\ 
J152356.26+034457.6  & 1.172 &52025-0592-443 &3.75  $\pm$0.65 & 364  & 0.39&-5888  & -4258  &-5135  &12.6 &T06 \\ 
J152438.79+415543.0  & 1.230 &53433-1678-106 &45.73 $\pm$2.75 & 4552 & 0.59&-30388 & -14544 &-21195 &16.8 &G09,Z10  \\ 
J153036.83+370439.2  & 0.417 &53144-1401-367 &19.84 $\pm$0.75 & 2082 & 0.58&-8707  & -1647  &-4467  &16.1 &G09,Z10  \\ 
J153133.53+452841.6  & 1.022 &52781-1332-245 &5.93  $\pm$0.94 & 431  & 0.53&-1314  & 480    &-420   &8.3  &T06 \\ 
J153646.88+515755.2  & 1.132 &52378-0795-095 &17.76 $\pm$0.87 & 1910 & 0.82&-7807  & -2717  &-4945  &13.4 &T06,G09,Z10   \\ 
J155905.39+250047.2  & 0.933 &53523-1655-085 &7.00  $\pm$0.75 & 736  & 0.58&-2256  & -192   &-1337  &9.1  &Z10 \\ 
J160018.68+021331.3  & 1.191 &52023-0595-041 &7.89  $\pm$2.04 & 815  & 0.91&-5272  & -2134  &-3532  &4.7  &G09 \\ 
J160329.72+502722.2  & 0.638 &52375-0620-126 &7.03  $\pm$0.83 & 740  & 0.49&-4836  & -2174  &-3567  &8.4  &T06,G09,Z10   \\ 
J160628.06+290333.8  & 0.434 &53496-1578-115 &3.10  $\pm$0.85 & 332  & 0.23&-3200  & -867   &-1990  &12.6 &Z10 \\ 
J160721.27+515510.6  & 0.776 &52375-0620-637 &6.12  $\pm$0.97 & 814  & 0.45&-7292  & -3220  &-5405  &10.2 &T06,Z10  \\ 
J161425.17+375210.7  & 0.553 &52764-1056-569 &3.01  $\pm$0.39 & 323  & 0.19&-6643  & -3929  &-5375  &30.9 &T06 \\ 
J161500.79+491045.4  & 1.280 &52054-0622-607 &5.87  $\pm$0.93 & 582  & 0.30&-6480  & -3082  &-4788  &13.5 &T06 \\ 
J161515.58+465931.9  & 0.986 &52377-0624-377 &8.47  $\pm$0.75 & 912  & 0.46&-6213  & -2605  &-4269  &14.1 &T06,G09,Z10   \\ 
J161740.36+421357.9  & 1.285 &52753-1171-447 &3.39  $\pm$0.65 & 452  & 0.32&-6125  & -2927  &-4422  &13.8 &T06 \\ 
J162016.29+415744.1  & 1.286 &52753-1171-603 &8.25  $\pm$0.70 & 882  & 0.52&-2976  & -365   &-1619  &12.5 &T06,Z10,G09,T06    \\ 
J162639.79+270155.5a & 0.826 &52822-1408-176 &2.01  $\pm$0.75 & 211  & 0.30&-4340  & -2770  &-3634  &7.5  &T06 \\ 
J162639.79+270155.5b & 0.826 &52822-1408-176 &3.91  $\pm$0.95 & 347  & 0.36&-6646  & -4748  &-5796  &7.5  &T06 \\ 
J162653.20+325406.3  & 0.951 &52520-1058-289 &3.57  $\pm$1.21 & 325  & 0.30&-3954  & -1971  &-3003  &8.5  &Z10 \\ 
J163255.46+420407.8  & 0.728 &52379-0816-569 &5.20  $\pm$0.85 & 551  & 0.40&-3236  & -559   &-2016  &10.7 &T06,Z10,T06   \\ 
J163513.51+213859.6  & 0.683 &53174-1571-121 &9.53  $\pm$1.33 & 1003 & 0.32&-8886  & -2722  &-5784  &8.5  &Z10 \\ 
J163656.84+364340.4  & 0.852 &52782-1174-337 &23.06 $\pm$0.87 & 2463 & 0.90&-7303  & -2684  &-4748  &8.1  &T06,G09,Z10   \\ 
J163825.67+462934.7  & 1.219 &52144-0627-137 &18.21 $\pm$1.02 & 1881 & 0.43&-15475 & -7773  &-11533 &16.0 &T06,G09,Z10   \\ 
J164447.19+311437.2  & 0.690 &52781-1340-002 &4.21  $\pm$0.65 & 464  & 0.33&-4770  & -1695  &-3459  &11.9 &T06 \\ 
J164721.01+410659.3  & 0.918 &52050-0630-455 &4.37  $\pm$0.91 & 418  & 0.28&-5987  & -3608  &-4868  &11.4 &T06,G09,Z10   \\ 
J164745.04+355732.9  & 0.942 &52409-0819-299 &5.56  $\pm$0.98 & 600  & 0.53&-2550  & -74    &-1077  &8.9  &T06 \\ 
J165225.39+215830.7  & 0.447 &52885-1415-231 &15.69 $\pm$1.80 & 1523 & 0.60&-8132  & -3731  &-6020  &4.9  &Z10 \\ 
J165236.27+190526.3  & 1.090 &53172-1567-341 &5.46  $\pm$1.22 & 634  & 0.57&-5849  & -3195  &-4614  &5.3  &G09 \\ 
J165238.29+414035.4  & 0.844 &52079-0631-181 &12.70 $\pm$0.69 & 1137 & 0.97&-2548  & 827    &-468   &5.5  &T06,T06  \\ 
J170010.82+395545.8  & 0.577 &52079-0633-482 &5.10  $\pm$1.26 & 688  & 0.35&-6974  & -3172  &-4896  &6.7  &T06,Z10  \\ 
J170330.23+324201.8  & 0.636 &52426-0973-108 &4.33  $\pm$1.06 & 520  & 0.36&-2782  & -170   &-1612  &7.7  &T06 \\ 
J170341.82+383944.7  & 0.554 &52071-0632-632 &11.53 $\pm$1.45 & 1139 & 0.54&-4954  & -229   &-2944  &5.8  &T06,Z10  \\ 
J171032.23+214451.3  & 0.867 &53177-1689-069 &9.95  $\pm$0.62 & 1064 & 0.73&-2623  & 336    &-1451  &11.7 &Z10 \\ 
J172042.43+273455.1  & 1.230 &52431-0980-165 &4.12  $\pm$1.60 & 438  & 0.59&-5331  & -3357  &-4379  &5.5  &T06 \\ 
J204333.20-001104.2  & 0.544 &52435-0981-044 &22.98 $\pm$1.03 & 2443 & 0.83&-10388 & -2069  &-5076  &13.8 &T06,G09,Z10   \\ 
J210704.93-011044.0  & 1.348 &52431-0985-124 &3.74  $\pm$1.03 & 396  & 0.28&-6078  & -3222  &-4655  &13.6 &G09,Z10  \\ 
J210757.67-062010.6  & 0.644 &52174-0637-610 &13.26 $\pm$0.43 & 1213 & 0.80&-2597  & 846    &-820   &25.7 &T06,G09,Z10   \\ 
J212017.00+004841.7  & 1.288 &52523-0987-408 &4.27  $\pm$0.41 & 449  & 0.20&-8578  & -5135  &-6840  &28.5 &T06,Z10,G09   \\ 
J214118.78-070957.4  & 0.869 &52824-1177-484 &11.98 $\pm$1.55 & 1028 & 0.74&-4431  & -1902  &-3021  &6.9  &T06,G09,Z10   \\ 
J220601.82-073312.1  & 0.900 &52468-0717-580 &12.68 $\pm$0.77 & 1345 & 0.83&-3100  & -629   &-1833  &7.7  &T06,G09,Z10   \\ 
J220931.92+125814.5  & 0.814 &52519-0735-501 &25.11 $\pm$0.97 & 2359 & 0.47&-12000 & -3931  &-7869  &14.5 &T06,G09,Z10   \\ 
J222609.49+010600.9  & 0.986 &52873-1103-601 &12.83 $\pm$1.19 & 1318 & 0.91&-2373  & 173    &-1139  &3.3  &G09 \\ 
J223424.10+005227.1  & 0.884 &52143-0376-615 &9.29  $\pm$0.96 & 869  & 0.34&-8377  & -3775  &-6042  &10.9 &T06,G09,Z10   \\ 
J224028.14-003813.1  & 0.658 &53261-1901-298 &15.69 $\pm$0.91 & 1718 & 0.79&-4601  & -77    &-1780  &21.7 &G09,Z10  \\ 
J232353.72-085857.9  & 0.807 &52203-0645-620 &6.89  $\pm$1.99 & 598  & 0.44&-5547  & -2891  &-4064  &6.4  &T06 \\ 
J232550.73-002200.4  & 1.011 &51818-0383-142 &9.50  $\pm$0.56 & 1038 & 0.58&-3887  & -872   &-2302  &17.5 &T06,G09,Z10   \\ 
J233635.75-010733.7  & 1.303 &51821-0384-011 &4.80  $\pm$0.96 & 435  & 0.27&-6571  & -3992  &-5268  &11.9 &T06 \\ 
J234157.24-094616.9  & 1.340 &52553-0647-036 &2.72  $\pm$0.82 & 286  & 0.23&-6763  & -4662  &-5833  &15.8 &T06 \\ 
J235718.32-090314.2  & 1.179 &52143-0650-321 &28.07 $\pm$3.77 & 2701 & 0.77&-18446 & -11556 &-14539 &7.3  &T06 \\ 
J235843.48+134200.2  & 1.135 &52235-0750-202 &6.89  $\pm$0.71 & 724  & 0.37&-11229 & -7549  &-9318  &14.2 &T06,G09,Z10   \\
\enddata
\tablenotetext{a}{The SDSS designation, hhmmss.ss+ddmmss.s (J2000). Sources with the same designation but postfixed with a/b/c
  denote sources with multiple Mg\,II absorption components.}
\tablenotetext{b}{The SDSS spectra are designated as mjd-plate-fiberid.} 
\tablenotetext{c}{The total error $\sigma_{\rm total}$ as defined in \S2.2\,.}
\tablenotetext{d}{Absorption Index (AI) measured according to the definition of Zhang \etal\  (2010).}
\tablenotetext{e}{Maximum depth of Mg\,II absorption troughs.}
\tablenotetext{f}{Maximum velocity of Mg\,II absorption troughs from the zero velocity.}
\tablenotetext{g}{Minimum velocity of Mg\,II absorption troughs from the zero velocity.}
\tablenotetext{h}{Weighted average velocity of Mg\,II BAL troughs.}
\tablenotetext{i}{Median signal to noise (S/N) in the range 2400--3000~\AA.}

{\it (This table is available in its entirety in a machine-readable form in the online
journal. A portion is shown here for guidance regarding its form and content.)}

%%\tablerefs{}
\end{deluxetable}
\end{landscape}



==> table8_complete.tex <==
\begin{landscape}
\pagestyle{empty}
\begin{deluxetable}{lrrrrrrrrrr}
\centering
\tablewidth{0pc}
\tablecolumns{11}
\tabletypesize{\footnotesize}
\tablecaption{UV continuum and emission-line parameters of the entire parent sample \label{tab:uvpar}}
\tablehead{
  \colhead{SDSS Name}  & \colhead{$z$} &
  \colhead{$\beta_{[3k-4k]}$}  & \colhead{log$L3000$} & \colhead{log$F_{2500}$} & \colhead{log$F$(UV Fe\,II)} &
  \colhead{FWHM(Mg\,II$^{b}$)} & \colhead{log$F$(Mg\,II$^{b})$} & \colhead{log$F$(Mg\,II$^{n})$} &
  \colhead{log$M_{BH}$} & \colhead{$L/L_{Edd}$} \\
  \colhead{}            & \colhead{}     &
  \colhead{}            & \colhead{erg~s$^{-1}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$ \AA$^{-1}$} &
  \colhead{ergs~s$^{-1}$~cm$^{-2}$}&
  \colhead{km~s$^{-1}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$} &
  \colhead{$\msun$} & \colhead{} }
\startdata
 J000009.26+151754.5 & 1.197 & -1.30 & 45.40 & -15.93 & -14.40 & 2435 & -14.68 & -15.61 & 8.38 & 0.51\\
 J002623.78+135523.5 & 1.319 & 5.03  & 45.39 & -15.95 & -13.47 & 2812 & -14.38 & -15.92 & 8.50 & 0.46\\
 J004610.17+000449.7 & 0.826 & -1.65 & 44.96 & -15.93 & -14.48 & 7771 & -14.39 &        & 9.16 & 0.03\\
 J005722.48+010101.8 & 1.146 & -1.27 & 45.52 & -15.74 & -13.91 & 3239 & -14.36 & -15.94 & 8.69 & 0.33\\
 J010352.46+003739.7 & 0.705 & -0.75 & 45.43 & -15.34 & -13.08 & 2747 & -13.66 & -15.77 & 8.50 & 0.39\\
 J011117.34+142653.6 & 1.155 & -0.25 & 45.76 & -15.64 & -13.77 & 4131 & -14.19 & -15.91 & 9.03 & 0.20\\
 J013816.16+140431.6 & 0.877 & -1.17 & 44.93 & -15.98 & -13.97 &      &        & -16.69 &      &     \\
 J013853.94-101125.7 & 1.305 & -1.56 & 45.47 & -15.90 & -13.69 & 2081 & -14.39 & -15.53 & 8.28 & 0.84\\
 J014012.07+130241.8 & 1.188 &       & 45.20 & -15.98 & -13.90 & 3036 & -14.65 & -15.76 & 8.47 & 0.35\\
 J014534.36+143136.9 & 0.636 & -0.94 & 44.63 & -15.99 & -13.93 & 1984 & -14.93 &        & 7.80 & 0.35\\
 J014950.96-010314.1 & 1.082 & -1.44 & 45.85 & -15.26 & -13.14 & 2622 & -14.01 &        & 8.68 & 0.90\\
 J015636.03+135212.3 & 1.129 & -1.40 & 45.40 & -15.90 & -13.59 & 3055 & -14.25 & -16.12 & 8.58 & 0.29\\
 J020105.14+000617.9 & 1.205 & -2.23 & 45.88 & -15.40 & -13.66 & 6453 & -13.88 & -16.33 & 9.48 & 0.14\\
 J023102.49-083141.2 & 0.587 & -1.70 & 44.83 & -15.65 & -13.49 & 2755 & -14.36 & -15.60 & 8.19 & 0.25\\
 J023153.64-093333.6 & 0.555 & -0.74 & 44.55 & -15.96 & -14.20 & 4724 & -14.83 & -16.22 & 8.51 & 0.05\\
 J023445.76-085908.5 & 1.275 & -1.44 & 45.33 & -16.05 & -13.95 & 3183 & -14.49 & -16.06 & 8.58 & 0.28\\
 J024220.10-085332.7 & 0.800 & -1.62 & 45.10 & -15.75 & -13.82 & 3871 & -14.27 & -15.97 & 8.63 & 0.16\\
 J024254.66-072205.6 & 1.217 & -1.36 & 45.49 & -15.85 & -13.74 & 5160 & -14.09 & -15.39 & 9.08 & 0.13\\
 J025026.66+000903.3 & 0.597 & 1.08  & 44.41 & -16.31 & -14.05 & 862  & -14.95 &        & 6.96 & 1.00\\
 J025204.17+010710.5 & 1.223 & 1.55  & 44.97 & -16.43 & -14.06 & 4031 & -14.91 & -16.09 & 8.59 & 0.10\\
 J025754.90-072449.5 & 1.023 & -1.56 & 45.35 & -15.77 & -13.90 & 3493 & -14.18 & -15.12 & 8.67 & 0.25\\
 J025813.67-011347.2 & 1.165 & -2.64 & 45.27 & -15.98 & -13.84 & 2951 & -14.61 &        & 8.48 & 0.33\\
 J033438.28-071149.0 & 0.635 & -1.90 & 45.55 & -15.01 & -12.82 & 3849 & -13.50 & -14.88 & 8.86 & 0.29\\
 J073122.84+430241.0 & 0.975 & -0.80 & 45.17 & -15.93 & -13.90 & 7095 & -14.44 & -15.64 & 9.19 & 0.05\\
 J074554.74+181817.0 & 1.054 & -0.74 & 45.44 & -15.79 & -13.75 & 2843 & -14.47 & -16.47 & 8.54 & 0.36\\
 J075325.52+414842.9 & 1.349 & -0.79 & 45.58 & -15.86 & -13.92 & 2176 & -14.66 & -15.68 & 8.38 & 0.79\\
 J075927.12+363431.5 & 0.983 & -0.47 & 45.18 & -15.98 & -13.92 & 1858 & -14.58 & -15.93 & 8.03 & 0.61\\
 J080248.19+551328.8 & 0.664 & 0.95  & 45.02 & -15.81 & -13.80 & 1634 & -14.44 &        & 7.84 & 0.54\\
 J080525.11+274321.8 & 0.895 & -1.04 & 44.97 & -16.03 & -14.12 & 6835 & -14.51 & -15.91 & 9.05 & 0.04\\
 J080559.43+563025.8 & 0.982 & -0.80 & 45.19 & -15.93 & -13.88 & 2284 & -14.60 & -16.61 & 8.22 & 0.44\\
 J080934.64+254837.9 & 0.545 & -1.78 & 45.24 & -15.13 & -13.46 & 5940 & -13.90 &        & 9.07 & 0.09\\
 J080957.38+181804.4 & 0.973 & -1.28 & 45.79 & -15.28 & -13.33 & 5904 & -13.44 &        & 9.35 & 0.13\\
 J081312.61+432640.1 & 1.090 & -2.03 & 45.38 & -15.79 & -14.10 & 5912 & -14.31 & -16.46 & 9.14 & 0.10\\
 J081314.80+385720.4 & 0.925 & -1.18 & 45.04 & -15.97 & -13.78 & 2088 & -14.85 & -16.29 & 8.06 & 0.50\\
 J081655.34+074311.5 & 0.645 & -1.25 & 44.96 & -15.67 & -13.77 & 3000 & -14.35 & -16.28 & 8.33 & 0.22\\
 J081819.29+562307.6 & 0.989 & -1.01 & 45.42 & -15.72 & -13.59 & 5159 & -14.09 & -15.31 & 9.04 & 0.11\\
 J081820.31+200046.1 & 0.986 & -1.55 & 45.37 & -15.65 & -13.51 & 3503 & -14.03 & -15.99 & 8.68 & 0.29\\
 J082052.63+401521.4 & 1.163 & -2.03 & 45.48 & -15.75 & -13.78 & 4682 & -14.36 & -15.62 & 8.99 & 0.17\\
 J082231.53+231152.0 & 0.653 & -1.38 & 45.47 & -15.16 & -14.11 & 7192 & -13.67 & -15.18 & 9.36 & 0.07\\
 J082525.52+352005.7 & 0.945 & -0.85 & 45.17 & -15.93 & -14.07 & 4153 & -14.58 & -16.41 & 8.72 & 0.13\\
 J083000.35+343238.7 & 0.740 & -1.23 & 44.89 & -15.91 & -14.15 & 3848 & -14.26 & -15.39 & 8.51 & 0.12\\
 J083522.77+424258.3 & 0.807 & -1.05 & 45.57 & -15.34 & -13.31 & 2074 & -14.04 & -15.74 & 8.33 & 0.83\\
 J083525.98+435211.3 & 0.568 & -1.28 & 45.20 & -15.25 & -12.97 & 6049 & -13.94 & -15.93 & 9.07 & 0.08\\
 J083613.23+280512.1 & 0.743 & -0.99 & 44.88 & -15.88 & -13.63 & 3352 & -14.58 &        & 8.39 & 0.17\\
 J084041.05+504107.7 & 1.130 & -1.64 & 45.37 & -15.82 & -13.70 & 5927 & -13.97 &        & 9.14 & 0.09\\
 J084044.41+363327.8 & 1.225 & -1.13 & 46.52 & -14.86 & -12.64 & 1983 & -13.40 &        & 8.78 & 2.51\\
 J084440.80+250253.2 & 1.001 & -1.18 & 45.36 & -15.71 & -13.59 & 3468 & -14.44 & -15.92 & 8.67 & 0.27\\
 J084638.50+225753.8 & 0.840 & -1.19 & 44.96 & -15.96 & -14.12 & 4214 & -14.60 &        & 8.63 & 0.11\\
 J084716.03+373218.0 & 0.453 & -1.72 & 44.74 & -15.46 & -13.41 & 2639 & -13.63 & -14.47 & 8.11 & 0.26\\
 J084824.14+034542.3 & 0.699 & -0.49 & 44.82 & -15.92 & -14.41 & 7207 & -14.43 & -15.55 & 9.02 & 0.03\\
 J084953.70+021709.4 & 1.112 & -1.19 & 45.29 & -15.91 & -14.08 & 7224 & -14.41 & -16.57 & 9.27 & 0.05\\
 J085007.76+081056.4 & 1.141 & -1.10 & 45.35 & -15.93 & -13.88 & 3316 & -14.42 & -15.45 & 8.63 & 0.26\\
 J085040.44+333500.6 & 1.055 & -1.77 & 45.15 & -16.06 & -13.76 & 2389 & -14.41 & -16.31 & 8.23 & 0.38\\
 J085053.12+445122.4 & 0.542 & -1.12 & 45.24 & -15.23 & -13.47 & 4639 & -13.97 & -16.06 & 8.86 & 0.12\\
 J085215.65+492040.8 & 0.567 & -1.16 & 44.74 & -15.72 & -14.90 & 4976 & -14.43 &        & 8.66 & 0.07\\
 J085357.88+463350.6 & 0.549 & -1.34 & 44.91 & -15.55 & -13.31 & 3267 & -14.06 & -15.24 & 8.38 & 0.18\\
 J090035.42+071811.9 & 1.210 & -1.47 & 45.36 & -15.91 & -13.75 & 2748 & -14.64 &        & 8.46 & 0.44\\
 J090056.89+021702.6 & 0.830 & -0.55 & 44.90 & -16.07 & -13.98 & 5614 & -14.26 & -16.28 & 8.85 & 0.05\\
 J090132.62+233257.7 & 0.845 & -1.50 & 45.16 & -15.74 & -13.70 & 3035 & -14.31 & -16.46 & 8.45 & 0.28\\
 J090154.96+380534.4 & 1.038 & -1.10 & 45.73 & -15.43 & -13.20 & 4589 & -14.02 & -15.27 & 9.10 & 0.21\\
 J090321.30+244928.0 & 1.235 & -1.33 & 45.08 & -16.20 & -14.15 & 6241 & -14.86 & -16.53 & 9.03 & 0.06\\
 J090825.06+014227.7 & 1.002 & -1.61 & 45.52 & -15.52 & -13.51 & 2432 & -14.34 & -16.41 & 8.44 & 0.72\\
 J091146.06+403501.0 & 0.441 & 0.33  & 44.44 & -15.86 & -13.62 & 1744 & -14.38 &        & 7.59 & 0.32\\
 J091214.02+424740.5 & 1.327 & -1.75 & 45.40 & -15.92 & -13.72 & 2705 & -14.55 & -15.77 & 8.47 & 0.54\\
 J091854.48+583339.6 & 1.315 & -0.44 & 45.37 & -16.11 & -15.21 & 6775 & -14.59 & -16.35 & 9.26 & 0.05\\
 J092035.59+524006.2 & 0.793 & 0.09  & 44.94 & -16.09 & -14.00 & 5609 & -14.32 & -16.25 & 8.87 & 0.04\\
 J092157.62+103539.0 & 0.548 & -1.02 & 44.68 & -15.68 & -13.62 & 3020 & -14.35 &        & 8.20 & 0.20\\
 J092441.08-001729.6 & 0.707 & -1.09 & 45.32 & -15.47 & -13.89 & 3208 & -14.04 & -14.92 & 8.58 & 0.25\\
 J092515.40+493539.8 & 1.294 & 2.17  & 45.59 & -15.76 & -13.86 & 4104 & -14.51 & -16.43 & 8.93 & 0.25\\
 J092928.63+324129.8 & 0.776 & -1.35 & 45.24 & -15.54 & -13.42 & 2517 & -14.15 & -15.50 & 8.33 & 0.47\\
 J093034.79+570520.6 & 0.637 & -1.65 & 45.00 & -15.58 & -13.44 & 2588 & -14.36 & -15.80 & 8.22 & 0.34\\
 J093228.56+555344.8 & 0.878 & -0.24 & 45.11 & -15.90 & -13.57 & 2281 & -14.27 & -15.93 & 8.17 & 0.40\\
 J093759.60+453801.8 & 0.429 & -1.47 & 44.67 & -15.50 & -13.96 & 7441 & -13.96 & -15.20 & 8.97 & 0.03\\
 J093919.87+440449.5 & 1.307 & 2.38  & 45.71 & -15.64 & -13.93 & 6733 & -14.37 & -15.63 & 9.43 & 0.11\\
 J093953.44+033229.7 & 0.927 & -0.61 & 45.06 & -15.94 & -13.74 & 1856 & -14.47 & -15.56 & 7.97 & 0.67\\
 J094225.42+565613.0 & 0.833 & -0.69 & 45.16 & -15.84 & -13.93 & 7236 & -14.17 & -16.02 & 9.20 & 0.04\\
 J094355.00+560649.0 & 1.055 & -0.37 & 45.25 & -15.99 & -14.12 & 2270 & -14.34 & -16.45 & 8.24 & 0.43\\
 J094443.13+062507.4 & 0.695 & -1.13 & 46.03 & -14.66 & -12.43 & 2195 & -13.45 &        & 8.62 & 1.41\\
 J094759.66+120537.7 & 1.287 & -1.34 & 45.44 & -15.93 & -13.67 & 2973 & -14.36 & -15.46 & 8.57 & 0.38\\
 J094939.93+393642.9 & 0.654 & -1.04 & 44.32 & -16.34 & -13.97 & 1135 & -14.88 &        & 7.16 & 0.74\\
 J095057.56+542919.4 & 1.194 & -2.11 & 45.22 & -16.04 & -14.24 & 1653 & -14.85 & -16.98 & 7.95 & 1.03\\
 J095914.91+131639.5 & 1.009 & -1.49 & 45.16 & -15.90 & -13.59 & 1727 & -14.44 & -16.07 & 7.96 & 0.93\\
 J100552.24+025902.4 & 0.908 & -1.50 & 45.32 & -15.69 & -13.79 & 5910 & -14.06 & -15.44 & 9.11 & 0.08\\
 J101139.21+415639.7 & 1.201 & -1.15 & 44.92 & -16.35 & -14.34 & 4437 & -14.87 & -16.39 & 8.65 & 0.10\\
 J101151.95+542942.6 & 0.536 & -0.93 & 44.30 & -16.17 & -14.59 & 2110 & -14.78 & -16.44 & 7.68 & 0.20\\
 J101203.31+492148.2 & 0.748 & -1.72 & 45.20 & -15.54 & -13.68 & 6211 & -14.41 &        & 9.09 & 0.07\\
 J101302.06+361510.7 & 0.836 & -1.21 & 44.89 & -15.99 & -13.65 & 1913 & -14.53 &        & 7.91 & 0.53\\
 J102021.21+121909.1 & 0.480 & 0.17  & 44.57 & -15.77 & -13.49 & 1384 & -14.57 &        & 7.46 & 0.63\\
 J102036.10+602339.0 & 0.994 & -0.51 & 45.30 & -15.98 & -14.45 &      &        &        &      &     \\
 J102225.67+602630.2 & 1.173 & -1.45 & 45.50 & -15.78 & -13.94 & 5053 & -14.44 & -15.58 & 9.07 & 0.14\\
 J102249.27+130125.0 & 1.217 & 0.08  & 45.35 & -16.07 & -13.76 & 2256 & -14.87 &        & 8.29 & 0.46\\
 J102802.33+592906.7 & 0.536 & -1.98 & 44.74 & -15.58 & -13.49 & 3400 & -14.06 & -15.78 & 8.33 & 0.17\\
 J102839.11+450009.4 & 0.585 & -0.95 & 45.43 & -15.05 & -12.78 & 2169 & -13.90 & -14.85 & 8.30 & 0.79\\
 J102943.75+370127.2 & 1.344 & -1.80 & 45.04 & -16.34 & -14.43 & 5751 & -14.57 & -16.36 & 8.94 & 0.07\\
 J103036.93+312028.8 & 0.876 & -1.30 & 45.62 & -15.34 & -13.31 & 6227 & -13.80 &        & 9.31 & 0.10\\
 J103110.64+395322.3 & 1.081 & -1.48 & 45.63 & -15.49 & -13.45 & 2004 & -14.56 &        & 8.33 & 1.20\\
 J103113.38+344613.5 & 0.942 & -1.55 & 45.32 & -15.72 & -13.73 &      &        & -15.69 &      &     \\
 J103255.37+083503.2 & 0.894 & -0.79 & 45.66 & -15.33 & -13.23 & 3103 & -13.65 & -16.31 & 8.73 & 0.42\\
 J103621.60+393701.6 & 0.802 & -1.06 & 45.71 & -15.12 & -12.90 & 2272 & -14.07 & -15.19 & 8.48 & 0.94\\
 J103739.61+501505.7 & 0.947 & -1.22 & 45.36 & -15.67 & -14.09 & 1403 & -15.08 &        & 7.88 & 1.59\\
 J103824.47-010538.9 & 0.773 & 1.16  & 44.63 & -16.38 & -14.31 & 5003 & -14.66 & -16.11 & 8.60 & 0.04\\
 J103929.00+472436.9 & 1.110 & 0.39  & 45.32 & -15.90 & -14.03 & 3102 & -14.70 & -16.47 & 8.55 & 0.30\\
 J103933.38+035200.4 & 0.916 & -0.57 & 44.84 & -16.23 & -13.91 & 2565 & -14.87 & -16.62 & 8.14 & 0.23\\
 J104035.07+623329.5 & 1.174 & -1.12 & 45.36 & -15.90 & -14.34 & 7100 & -14.59 & -16.36 & 9.29 & 0.06\\
 J104116.79+035511.4 & 1.246 & -0.96 & 45.54 & -15.81 & -13.78 & 2103 & -14.45 & -15.69 & 8.33 & 0.82\\
 J104132.96+513657.0 & 0.735 & -1.53 & 45.30 & -15.47 & -13.42 & 4468 & -14.00 & -16.03 & 8.86 & 0.15\\
 J104210.43+501609.1 & 0.789 & -1.22 & 45.44 & -15.38 & -13.45 & 5533 & -14.15 &        & 9.12 & 0.11\\
 J104459.60+365605.1 & 0.701 & -1.10 & 45.75 & -15.00 & -12.79 & 940  & -14.12 &        & 7.74 & 4.99\\
 J104705.08+590728.4 & 0.392 & -1.83 & 44.44 & -15.62 & -13.80 & 2014 & -14.50 & -15.36 & 7.72 & 0.32\\
 J104838.65+603933.1 & 1.274 & -1.86 & 45.35 & -16.00 & -13.95 & 7061 & -14.55 & -15.96 & 9.28 & 0.06\\
 J104845.83+353110.7 & 1.011 & -1.34 & 45.85 & -15.23 & -13.66 & 2869 & -14.22 & -15.35 & 8.76 & 0.70\\
 J105102.78+525049.8 & 0.543 & -1.36 & 44.65 & -15.79 & -14.08 & 5598 & -14.21 & -16.18 & 8.72 & 0.05\\
 J105259.99+065358.0 & 0.724 & -0.97 & 44.86 & -15.89 & -13.29 & 2349 & -14.25 &        & 8.07 & 0.32\\
 J105404.72+042939.3 & 0.579 & -1.24 & 44.58 & -15.98 & -13.99 & 5335 & -14.69 & -16.25 & 8.64 & 0.04\\
 J105638.08+494943.3 & 1.148 & -1.96 & 46.24 & -14.97 & -13.16 & 4909 & -13.50 & -15.04 & 9.43 & 0.36\\
 J105748.63+610910.8 & 1.274 & -1.96 & 45.10 & -16.30 & -14.13 & 4261 & -14.61 & -16.03 & 8.71 & 0.12\\
 J105823.13+600805.6 & 1.071 & -0.97 & 45.61 & -15.56 & -13.54 & 2088 & -14.21 & -15.26 & 8.35 & 0.95\\
 J110108.43+515021.9 & 0.968 & -1.53 & 45.69 & -15.35 & -13.23 & 3691 & -13.87 & -14.90 & 8.89 & 0.34\\
 J110440.82-000441.6 & 1.344 & 1.82  & 45.45 & -15.93 & -13.77 & 2176 & -14.69 &        & 8.31 & 0.79\\
 J110810.99+352927.4 & 1.062 & -1.02 & 45.08 & -16.04 & -13.79 & 1227 & -14.58 & -16.13 & 7.62 & 1.66\\
 J110839.62+532721.4 & 0.878 & -0.33 & 44.87 & -16.18 & -14.12 & 3323 & -14.87 &        & 8.38 & 0.13\\
 J111013.79+523607.2 & 1.009 & -1.37 & 45.78 & -15.27 & -13.08 & 2352 & -13.95 & -15.68 & 8.55 & 1.01\\
 J111040.48+433821.3 & 1.230 & -2.38 & 45.37 & -15.91 & -13.66 & 5128 & -14.31 & -16.78 & 9.01 & 0.13\\
 J111628.00+434505.8 & 0.801 & -0.90 & 45.60 & -15.28 & -13.17 & 2691 & -14.08 & -15.78 & 8.57 & 0.53\\
 J112349.16+135220.6 & 0.928 & -1.15 & 44.32 & -16.00 & -13.92 & 7041 & -14.58 & -16.74 & 8.74 & 0.02\\
 J112632.81+430938.5 & 0.436 & 0.19  & 44.65 & -15.66 & -13.62 & 941  & -14.64 & -16.86 & 7.16 & 1.32\\
 J112730.71+423039.0 & 0.531 & -1.56 & 44.66 & -15.73 & -14.05 & 3029 & -14.44 & -15.58 & 8.19 & 0.17\\
 J112822.42+482310.1 & 0.541 & -0.60 & 45.15 & -15.33 & -13.21 & 2561 & -14.32 &        & 8.30 & 0.35\\
 J112828.31+011337.9 & 0.893 & -0.66 & 45.25 & -15.85 & -14.27 &      &        &        &      &     \\
 J112901.71+050617.0 & 1.282 & 0.82  & 45.25 & -16.24 & -14.02 & 3311 & -14.61 & -16.59 & 8.57 & 0.19\\
 J112912.27+422853.9 & 0.582 & -0.64 & 44.82 & -15.74 & -13.55 & 1989 & -14.26 & -15.33 & 7.90 & 0.40\\
 J113349.81+361027.3 & 1.158 & -0.40 & 45.22 & -16.13 & -13.89 & 2219 & -14.59 &        & 8.21 & 0.44\\
 J113355.22+111208.8 & 0.763 & -1.50 & 45.02 & -15.72 & -13.49 & 2461 & -14.50 &        & 8.19 & 0.41\\
 J113704.85+055240.4 & 0.915 & -1.48 & 45.99 & -16.36 &        &      &        &        &      &     \\
 J113807.83+531231.6 & 0.790 & -1.31 & 45.24 & -15.60 & -13.82 & 2163 & -14.67 &        & 8.19 & 0.59\\
 J113940.42+451207.0 & 1.141 & -1.43 & 45.57 & -15.64 & -13.42 & 2940 & -14.28 &        & 8.63 & 0.47\\
 J114033.47+150701.7 & 1.250 & -1.25 & 45.57 & -15.78 & -14.37 & 3177 & -14.69 & -15.83 & 8.70 & 0.38\\
 J114043.62+532438.9 & 0.530 & -1.39 & 44.87 & -15.57 & -14.04 & 2222 & -14.30 & -16.50 & 8.02 & 0.35\\
 J114111.61-014306.6 & 1.266 & -1.49 & 45.99 & -15.37 & -13.30 & 3183 & -14.15 & -15.21 & 8.92 & 0.61\\
 J114209.01+070957.7 & 0.497 & -1.41 & 44.77 & -15.52 & -13.28 & 4204 & -14.36 & -15.60 & 8.53 & 0.10\\
 J114516.73+493259.4 & 1.158 & -0.73 & 45.57 & -15.74 & -13.65 & 5407 & -14.31 & -16.48 & 9.16 & 0.12\\
 J114600.32+504734.0 & 1.084 & -1.58 & 45.50 & -15.60 & -13.60 & 3790 & -14.49 &        & 8.82 & 0.30\\
 J114740.33+373438.9 & 1.297 & 2.04  & 45.20 & -16.28 & -13.81 & 3221 & -14.69 & -15.96 & 8.52 & 0.20\\
 J114754.36+040638.4 & 1.174 & -2.50 & 45.30 & -15.92 & -14.01 & 5004 & -14.37 & -15.78 & 8.96 & 0.13\\
 J114915.30+393325.4 & 0.630 & -0.91 & 44.75 & -15.81 & -13.71 & 1231 & -14.62 &        & 7.45 & 1.15\\
 J115010.81+480844.3 & 1.190 & -3.60 & 45.37 & -15.85 & -13.80 & 2954 & -14.55 & -16.22 & 8.53 & 0.42\\
 J115511.93+465903.7 & 1.298 & -2.37 & 45.65 & -15.72 & -13.65 & 4560 & -14.67 &        & 9.05 & 0.21\\
 J115553.87+012427.6 & 1.010 & -1.09 & 45.58 & -15.54 & -13.66 & 2571 & -14.25 &        & 8.52 & 0.58\\
 J115816.72+132624.1 & 0.440 & -1.18 & 45.04 & -15.14 & -12.99 & 2520 & -13.80 &        & 8.22 & 0.38\\
 J115832.28+044208.3 & 0.896 & -2.08 & 45.44 & -15.50 & -13.28 & 3913 & -14.03 & -15.03 & 8.82 & 0.24\\
 J115852.87-004301.9 & 0.983 & -0.24 & 45.01 & -16.16 & -13.93 & 5196 & -14.44 & -15.82 & 8.84 & 0.06\\
 J115923.83+415246.7 & 1.200 & -1.69 & 45.89 & -15.39 & -13.45 & 4493 & -14.04 & -15.26 & 9.17 & 0.28\\
 J120049.55+632211.8 & 0.887 & -0.48 & 45.01 & -16.03 & -13.84 & 7096 & -14.60 &        & 9.11 & 0.03\\
 J120146.46+630034.4 & 0.659 & -1.60 & 44.83 & -15.85 & -14.60 & 6381 & -14.42 & -16.47 & 8.92 & 0.04\\
 J120337.91+153006.6 & 1.218 & -1.37 & 45.83 & -15.60 & -13.65 & 6840 & -13.96 & -15.51 & 9.50 & 0.08\\
 J120813.42+023015.1 & 1.182 & -1.36 & 46.45 & -14.78 & -12.61 & 2074 & -13.44 & -14.33 & 8.79 & 2.69\\
 J120924.07+103612.0 & 0.395 & -1.71 & 45.50 & -14.61 & -13.10 & 6339 & -13.23 & -15.46 & 9.27 & 0.09\\
 J120928.11+003511.6 & 0.610 & 1.62  & 44.09 & -16.56 & -14.41 & 717  & -15.89 &        & 6.64 & 1.22\\
 J121113.38+121937.3 & 0.465 & -0.47 & 44.72 & -15.56 & -13.31 & 2183 & -14.18 &        & 7.93 & 0.32\\
 J121303.40-014450.9 & 0.613 & -1.04 & 45.04 & -15.54 & -13.64 & 2350 & -14.46 & -15.90 & 8.16 & 0.39\\
 J121441.42-000137.8 & 1.046 & -0.87 & 44.88 & -16.33 & -13.49 & 4425 & -14.50 & -15.70 & 8.63 & 0.08\\
 J121806.00+101920.6 & 1.089 & 0.09  & 45.06 & -16.25 & -14.29 & 8289 & -14.61 & -16.12 & 9.27 & 0.02\\
 J121907.80-005609.2 & 0.638 & 0.42  & 44.46 & -16.28 & -14.00 & 1563 & -14.87 & -16.41 & 7.51 & 0.36\\
 J122020.29+575637.6 & 1.307 & 2.18  & 45.14 & -16.37 & -14.19 & 2063 & -14.76 & -16.54 & 8.10 & 0.43\\
 J122043.21-013215.3 & 0.448 & -0.95 & 44.26 & -16.01 & -14.43 & 4242 & -14.94 &        & 8.27 & 0.05\\
 J122305.79+085651.4 & 1.091 & -1.71 & 45.46 & -15.70 & -13.71 & 3367 & -14.30 & -15.22 & 8.69 & 0.33\\
 J122424.17+593528.5 & 0.899 & -1.62 & 45.10 & -15.86 & -13.68 & 3730 & -14.33 & -16.19 & 8.60 & 0.18\\
 J122614.97+120925.4 & 0.871 & -1.11 & 45.47 & -15.58 & -13.94 & 2086 & -14.04 & -15.69 & 8.28 & 0.64\\
 J122703.19+505356.2 & 0.765 & 0.79  & 44.97 & -16.02 & -13.88 & 1193 & -14.70 & -15.86 & 7.54 & 0.94\\
 J122847.60+490431.8 & 0.954 & -0.87 & 45.13 & -15.90 & -13.80 & 2671 & -14.44 & -15.66 & 8.32 & 0.34\\
 J123218.09+410637.9 & 1.326 & -0.54 & 45.51 & -15.94 & -14.26 & 10330& -15.18 &        & 9.69 & 0.03\\
 J124300.87+153510.6 & 0.562 & -1.19 & 44.83 & -15.63 & -13.47 & 5470 & -14.04 & -15.84 & 8.79 & 0.06\\
 J125057.57+402100.2 & 0.607 & -0.75 & 44.62 & -15.98 & -14.07 & 1986 & -15.03 &        & 7.80 & 0.32\\
 J125507.12+634423.8 & 1.067 & -1.63 & 45.07 & -16.03 & -13.56 & 5005 & -14.51 & -15.94 & 8.84 & 0.10\\
 J130006.47+653201.7 & 1.192 & -0.93 & 45.39 & -15.88 & -14.06 & 4400 & -14.70 &        & 8.89 & 0.17\\
 J130444.12+052820.8 & 0.935 & -1.74 & 45.05 & -15.94 & -13.87 & 1087 & -14.52 & -15.79 & 7.50 & 2.00\\
 J130741.12+503106.4 & 0.695 & -0.73 & 45.17 & -15.59 & -13.48 & 6203 & -14.52 &        & 9.07 & 0.06\\
 J130952.89+011950.6 & 0.547 & -1.47 & 45.30 & -15.12 & -13.25 & 7927 & -13.55 & -14.65 & 9.35 & 0.05\\
 J131323.25+151309.6 & 1.262 & -1.49 & 46.00 & -15.32 & -13.35 & 4524 & -14.03 & -15.27 & 9.23 & 0.32\\
 J131433.19+471457.7 & 0.873 & -1.14 & 45.06 & -15.89 & -13.99 & 1261 & -15.03 & -16.43 & 7.63 & 1.38\\
 J131637.26-003636.0 & 0.930 & -1.42 & 45.52 & -15.48 & -13.40 & 11377& -13.91 & -15.66 & 9.78 & 0.03\\
 J131703.87+614228.5 & 1.344 & -0.55 & 45.39 & -16.07 & -14.04 & 5564 & -14.59 & -16.24 & 9.10 & 0.09\\
 J131823.73+123812.5 & 0.589 & -0.80 & 44.68 & -15.89 & -14.11 & 1235 & -14.81 &        & 7.41 & 0.88\\
 J132114.42+020225.0 & 0.582 & 0.29  & 44.47 & -16.06 & -13.28 & 2273 & -14.36 & -16.06 & 7.84 & 0.22\\
 J132401.53+032020.6 & 0.926 & -0.09 & 44.94 & -16.13 & -13.95 & 3231 & -14.12 & -15.95 & 8.39 & 0.16\\
 J132439.32+421604.7 & 1.020 & -1.03 & 45.19 & -15.97 & -14.46 & 7467 & -14.44 & -15.80 & 9.24 & 0.04\\
 J133014.48+413244.9 & 1.146 & -1.77 & 45.69 & -15.49 & -13.49 & 3105 & -14.08 &        & 8.74 & 0.54\\
 J133603.65+511733.6 & 1.327 & -0.54 & 45.44 & -15.93 & -13.88 & 2244 & -14.61 & -15.74 & 8.33 & 0.72\\
 J133833.82+034522.2 & 1.301 & 1.88  & 45.48 & -16.00 & -13.90 & 6872 & -14.98 &        & 9.32 & 0.06\\
 J133936.69+111949.2 & 0.650 & -0.71 & 44.87 & -15.77 & -13.52 & 1180 & -14.41 & -15.70 & 7.48 & 1.28\\
 J134127.40+002050.5 & 0.722 & -0.85 & 44.90 & -15.83 & -14.02 & 1877 & -14.58 & -15.47 & 7.89 & 0.56\\
 J134410.43+535352.8 & 0.827 & -2.40 & 45.24 & -15.61 & -13.90 & 5863 & -14.42 & -16.02 & 9.06 & 0.09\\
 J134415.75+331719.1 & 0.687 & -1.10 & 45.02 & -15.75 & -14.01 & 7014 & -14.25 & -15.49 & 9.10 & 0.04\\
 J134450.16-015843.0 & 0.958 & -1.17 & 45.10 & -15.91 & -13.71 & 1818 & -14.56 &        & 7.97 & 0.77\\
 J134830.78-015357.8 & 0.816 & -1.04 & 44.92 & -15.96 & -13.77 & 3640 & -14.38 & -16.54 & 8.48 & 0.14\\
 J134938.48+475530.1 & 1.104 & -1.34 & 45.75 & -15.43 & -13.33 & 3112 & -14.13 & -15.94 & 8.77 & 0.52\\
 J134951.56+040407.2 & 1.032 & -1.62 & 45.60 & -15.49 & -13.67 & 4542 & -14.24 & -15.50 & 9.02 & 0.22\\
 J135226.34+024549.4 & 1.222 & -1.57 & 45.55 & -15.75 & -13.91 & 5894 & -13.98 & -15.78 & 9.23 & 0.11\\
 J135418.26+585935.9 & 0.791 & -0.59 & 44.89 & -15.97 & -14.10 & 1296 & -15.02 &        & 7.57 & 1.07\\
 J135546.11+431819.8 & 1.318 & 0.59  & 45.59 & -15.77 & -13.77 & 6828 & -14.36 & -15.41 & 9.38 & 0.09\\
 J135750.89+632446.2 & 1.347 & -1.10 & 45.60 & -15.88 & -13.70 & 2441 & -14.34 & -15.50 & 8.49 & 0.59\\
 J140025.53-012957.0 & 0.584 & -0.68 & 44.82 & -15.74 & -13.47 & 7143 & -14.29 &        & 9.02 & 0.03\\
 J140115.74+621857.1 & 0.645 & 0.67  & 44.68 & -16.04 & -13.78 & 1860 & -14.59 &        & 7.77 & 0.34\\
 J140332.86+133218.7 & 1.093 & -1.30 & 45.59 & -15.61 & -13.59 & 4364 & -14.12 & -15.59 & 8.99 & 0.20\\
 J141513.20+634037.2 & 1.334 & -2.29 & 45.58 & -15.81 & -14.03 & 3924 & -14.53 & -15.66 & 8.89 & 0.27\\
 J141555.07+582632.8 & 1.261 & -1.63 & 45.52 & -15.85 & -14.39 & 3363 & -14.76 & -15.72 & 8.72 & 0.31\\
 J142010.28+604722.3 & 1.345 & -1.87 & 45.01 & -16.49 & -14.86 &      &        &        &      &     \\
 J142110.71+035439.8 & 0.831 & -1.09 & 44.68 & -16.20 & -14.03 & 2701 & -14.57 & -16.21 & 8.10 & 0.21\\
 J142116.23+052252.3 & 0.926 & -0.40 & 45.09 & -15.99 & -14.01 & 4005 & -14.80 &        & 8.65 & 0.12\\
 J142647.47+401250.8 & 0.749 & -1.54 & 44.97 & -15.77 & -13.85 & 2911 & -14.43 & -15.37 & 8.31 & 0.26\\
 J142649.24+032517.7 & 0.529 & -0.90 & 44.74 & -15.67 & -13.57 & 2944 & -14.32 & -16.06 & 8.20 & 0.19\\
 J142927.28+523849.5 & 0.595 & -0.90 & 45.34 & -15.20 & -12.89 & 1592 & -13.88 &        & 7.98 & 1.18\\
 J143144.91+391910.2 & 1.091 & -1.33 & 45.77 & -15.46 & -14.03 & 8879 & -14.07 & -15.37 & 9.70 & 0.06\\
 J143303.27+403105.1 & 0.446 & -1.55 & 44.59 & -15.61 & -13.55 & 2885 & -14.35 & -15.26 & 8.11 & 0.18\\
 J143826.73+642859.8 & 1.222 & -1.30 & 45.70 & -15.60 & -13.60 & 2079 & -14.31 & -15.88 & 8.40 & 1.08\\
 J143828.63+452108.6 & 0.427 & -1.51 & 44.79 & -15.34 & -13.27 & 1884 & -14.17 & -15.28 & 7.84 & 0.54\\
 J144222.02+524143.2 & 1.037 & -1.04 & 45.17 & -15.99 & -13.93 & 2680 & -14.71 & -15.81 & 8.35 & 0.33\\
 J144317.71-020933.0 & 1.050 & -0.83 & 45.40 & -15.82 & -14.04 & 3145 & -14.79 &        & 8.60 & 0.28\\
 J144342.21-025430.6 & 0.777 & -0.31 & 44.85 & -16.04 & -13.73 & 1263 & -14.74 &        & 7.53 & 0.95\\
 J144436.58+425508.6 & 1.101 & -1.50 & 45.43 & -15.69 & -13.54 & 4847 & -14.21 & -15.28 & 9.00 & 0.17\\
 J144627.41+353453.5 & 0.922 & -1.75 & 45.66 & -15.34 & -13.74 & 7358 & -14.00 & -15.17 & 9.48 & 0.08\\
 J144642.26+454630.9 & 0.738 & -1.04 & 45.05 & -15.82 & -14.25 & 1910 & -14.56 & -16.75 & 7.99 & 0.48\\
 J144759.19+350833.5 & 0.953 & -1.36 & 45.39 & -15.63 & -13.63 & 2752 & -14.31 & -15.40 & 8.48 & 0.45\\
 J144903.18+503018.1 & 0.609 & -1.43 & 44.82 & -15.73 & -13.78 & 2022 & -14.59 & -15.67 & 7.92 & 0.44\\
 J145333.01+002943.6 & 1.291 & -1.44 & 45.25 & -16.27 & -14.29 & 2602 & -15.02 & -16.15 & 8.36 & 0.29\\
 J145503.95+515539.8 & 1.277 & 0.36  & 45.32 & -16.11 & -14.12 & 2800 & -14.62 & -15.58 & 8.46 & 0.32\\
 J145549.84-013018.3 & 1.321 & 0.60  & 45.34 & -16.13 & -14.21 & 4302 & -14.60 & -16.22 & 8.85 & 0.14\\
 J145724.00+452157.8 & 0.718 & -1.19 & 44.96 & -15.79 & -13.32 & 2064 & -14.47 &        & 8.01 & 0.46\\
 J145736.70+523454.6 & 0.638 & -1.35 & 45.14 & -15.41 & -13.18 & 2305 & -14.00 &        & 8.20 & 0.53\\
 J145836.73+433015.5 & 0.760 & -1.22 & 45.10 & -15.72 & -13.81 & 4207 & -14.37 & -15.82 & 8.70 & 0.13\\
 J150525.51-023853.8 & 1.159 & -0.90 & 45.43 & -15.86 & -13.76 & 2617 & -14.42 & -15.83 & 8.46 & 0.46\\
 J150847.41+340437.7 & 0.788 & -1.27 & 45.64 & -15.21 & -14.17 & 8948 & -13.70 & -14.78 & 9.64 & 0.05\\
 J151053.63+574055.1 & 1.037 & -0.43 & 45.68 & -15.52 & -13.47 & 2359 & -13.97 & -15.28 & 8.50 & 0.67\\
 J151225.67+585752.2 & 0.791 & 1.96  & 44.40 & -16.63 & -14.35 & 1362 & -14.83 &        & 7.36 & 0.38\\
 J151545.34+031745.0 & 0.780 & -1.36 & 44.67 & -16.24 & -14.16 & 3317 & -14.54 &        & 8.27 & 0.11\\
 J151548.67+430420.5 & 0.527 & -0.55 & 44.32 & -16.13 & -13.87 & 2029 & -14.78 & -16.25 & 7.66 & 0.22\\
 J152200.76+035017.0 & 0.838 & -1.32 & 45.07 & -15.85 & -14.32 & 5324 & -14.84 & -16.26 & 8.89 & 0.08\\
 J152356.26+034457.6 & 1.172 & -1.67 & 45.44 & -15.78 & -13.64 & 2458 & -14.51 & -15.86 & 8.41 & 0.63\\
 J152438.79+415543.0 & 1.230 & -0.97 & 45.74 & -15.62 & -13.45 & 926  & -15.81 &        & 7.72 & 4.97\\
 J153036.83+370439.2 & 0.417 & -0.89 & 44.90 & -15.26 & -13.20 & 2138 & -13.85 &        & 8.01 & 0.42\\
 J153133.53+452841.6 & 1.022 & -0.85 & 45.19 & -15.97 & -13.99 & 7110 & -14.36 & -15.84 & 9.20 & 0.05\\
 J153646.88+515755.2 & 1.132 & -0.96 & 45.65 & -15.63 & -13.82 & 2992 & -14.28 & -16.39 & 8.69 & 0.42\\
 J155905.39+250047.2 & 0.933 & -1.41 & 45.29 & -15.70 & -13.77 & 2126 & -14.64 & -15.94 & 8.21 & 0.68\\
 J160018.68+021331.3 & 1.191 & -1.76 & 45.08 & -16.17 & -14.15 & 3082 & -15.11 &        & 8.42 & 0.26\\
 J160329.72+502722.2 & 0.638 & -1.29 & 44.81 & -15.81 & -13.98 & 2920 & -14.55 &        & 8.23 & 0.20\\
 J160628.06+290333.8 & 0.434 & 0.16  & 44.88 & -15.40 & -13.49 & 2140 & -14.10 & -15.18 & 8.00 & 0.34\\
 J160721.27+515510.6 & 0.776 & -1.91 & 44.98 & -15.81 & -13.80 & 2202 & -14.38 & -16.33 & 8.08 & 0.45\\
 J161425.17+375210.7 & 0.553 & -1.54 & 45.46 & -14.94 & -12.95 & 3331 & -13.59 & -14.64 & 8.68 & 0.36\\
 J161500.79+491045.4 & 1.280 & -0.85 & 45.45 & -15.91 & -13.76 & 2813 & -14.34 & -15.96 & 8.53 & 0.43\\
 J161515.58+465931.9 & 0.986 & -0.94 & 45.35 & -15.79 & -13.79 & 2480 & -14.39 & -15.45 & 8.37 & 0.44\\
 J161740.36+421357.9 & 1.285 & -2.25 & 45.66 & -15.68 & -13.74 & 3726 & -14.29 & -15.65 & 8.88 & 0.33\\
 J162016.29+415744.1 & 1.286 & -1.19 & 45.56 & -15.85 & -14.29 & 3089 & -14.14 & -16.18 & 8.67 & 0.36\\
 J162639.79+270155.5 & 0.826 & -1.43 & 44.99 & -15.87 & -13.93 & 3027 & -14.68 & -16.33 & 8.36 & 0.24\\
 J162653.20+325406.3 & 0.951 & -1.45 & 45.16 & -15.89 & -13.84 & 2940 & -14.37 &        & 8.42 & 0.28\\
 J163255.46+420407.8 & 0.728 & -1.28 & 44.93 & -15.89 & -14.34 & 7571 & -14.16 & -15.64 & 9.12 & 0.03\\
 J163513.51+213859.6 & 0.683 & -1.04 & 44.94 & -15.73 & -13.72 & 1556 & -14.46 & -15.94 & 7.75 & 0.85\\
 J163656.84+364340.4 & 0.852 & -0.31 & 45.10 & -15.90 & -13.72 & 1726 & -14.38 &        & 7.92 & 0.66\\
 J163825.67+462934.7 & 1.219 & -1.28 & 45.32 & -15.92 & -13.43 & 3193 & -14.10 &        & 8.57 & 0.34\\
 J164447.19+311437.2 & 0.690 & -0.88 & 45.23 & -15.54 & -13.41 & 2957 & -14.19 & -15.94 & 8.46 & 0.26\\
 J164721.01+410659.3 & 0.918 & -1.69 & 45.14 & -15.82 & -13.89 & 3940 & -14.46 & -16.29 & 8.66 & 0.17\\
 J164745.04+355732.9 & 0.942 & -1.89 & 45.08 & -15.92 & -13.77 & 958  & -14.91 &        & 7.40 & 2.70\\
 J165225.39+215830.7 & 0.447 & 0.23  & 44.46 & -15.83 & -13.61 & 1046 & -14.27 &        & 7.16 & 0.93\\
 J165236.27+190526.3 & 1.090 & -0.63 & 45.03 & -16.17 & -14.08 & 4294 & -14.31 & -15.57 & 8.68 & 0.11\\
 J165238.29+414035.4 & 0.844 & 0.28  & 44.83 & -16.23 & -14.40 & 3760 & -14.68 &        & 8.46 & 0.09\\
 J170010.82+395545.8 & 0.577 & -0.43 & 44.64 & -15.91 & -13.81 & 2051 & -14.80 &        & 7.83 & 0.31\\
 J170330.23+324201.8 & 0.636 & -1.49 & 44.66 & -15.95 & -13.72 & 3352 & -14.65 & -16.04 & 8.28 & 0.13\\
 J170341.82+383944.7 & 0.554 & 0.39  & 44.66 & -15.98 & -14.39 & 3074 & -14.53 & -16.37 & 8.20 & 0.10\\
 J171032.23+214451.3 & 0.867 & -1.06 & 45.13 & -15.85 & -14.05 & 1157 & -14.85 & -15.88 & 7.59 & 1.67\\
 J172042.43+273455.1 & 1.230 & -1.56 & 45.06 & -16.20 & -14.22 & 2298 & -15.04 &        & 8.15 & 0.48\\
 J204333.20-001104.2 & 0.544 & -0.70 & 45.09 & -15.34 & -13.37 & 2642 & -14.16 &        & 8.29 & 0.34\\
 J210704.93-011044.0 & 1.348 & -4.73 & 45.62 & -15.79 & -13.76 & 3857 & -14.28 & -16.26 & 8.89 & 0.28\\
 J210757.67-062010.6 & 0.644 & -0.64 & 45.40 & -15.31 & -13.25 & 4517 & -13.46 & -15.25 & 8.92 & 0.13\\
 J212017.00+004841.7 & 1.288 & -0.98 & 46.00 & -15.36 & -13.34 & 6054 & -13.82 & -14.82 & 9.48 & 0.17\\
 J214118.78-070957.4 & 0.869 & -0.28 & 44.84 & -16.21 & -14.26 & 2380 & -14.85 & -16.60 & 8.07 & 0.24\\
 J220601.82-073312.1 & 0.900 & -0.93 & 45.12 & -15.90 & -13.79 & 1989 & -14.77 & -16.05 & 8.06 & 0.57\\
 J220931.92+125814.5 & 0.814 & -0.85 & 45.24 & -15.62 & -13.35 & 2036 & -14.24 &        & 8.14 & 0.67\\
 J222609.49+010600.9 & 0.986 & 0.60  & 44.84 & -16.26 & -13.92 & 3361 & -14.46 & -15.97 & 8.37 & 0.15\\
 J223424.10+005227.1 & 0.884 & -1.05 & 45.23 & -15.73 & -13.50 & 3307 & -14.29 & -16.29 & 8.56 & 0.24\\
 J224028.14-003813.1 & 0.658 & -1.00 & 45.01 & -15.63 & -13.53 & 3805 & -14.19 &        & 8.57 & 0.15\\
 J232353.72-085857.9 & 0.807 & -1.08 & 44.80 & -16.12 & -13.96 & 4606 & -14.43 & -16.13 & 8.62 & 0.07\\
 J232550.73-002200.4 & 1.011 & -1.30 & 45.65 & -15.48 & -13.86 & 5367 & -14.06 & -15.33 & 9.20 & 0.14\\
 J233635.75-010733.7 & 1.303 & 1.82  & 45.45 & -15.96 & -14.15 & 1190 & -15.13 &        & 7.78 & 2.26\\
 J234157.24-094616.9 & 1.340 & -1.48 & 45.72 & -15.69 & -13.84 & 4309 & -14.42 & -16.51 & 9.04 & 0.25\\
 J235718.32-090314.2 & 1.179 & -1.50 & 45.31 & -15.92 & -14.44 & 3834 & -14.53 &        & 8.73 & 0.22\\
 J235843.48+134200.2 & 1.135 & -1.15 & 45.48 & -15.73 & -13.50 & 2430 & -14.31 & -15.54 & 8.42 & 0.63\\
{\it (This table is available in its entirety in a machine-readable form in the online
journal. A portion is shown here for guidance regarding its form and content.)}
\end{deluxetable}
\end{landscape}
\clearpage




==> table9_complete.tex <==
\begin{landscape}
\pagestyle{empty}
\begin{deluxetable}{lrrrrrrrrrr}
\centering
\tablewidth{0pc}
\tablecolumns{11}
\tabletypesize{\footnotesize}
\tablecaption{Optical continuum and emission-line parameters of the $z<0.8$ objects in the parent sample \label{tab:opticalpar}}
\tablehead{
  \colhead{SDSS NAME}  & \colhead{$z$} &
  \colhead{log$L5100$} & \colhead{$FWHM(\rm H\beta^{b}$} & \colhead{log$F(\rm H\beta^{b})$} &
  \colhead{log$F(\rm H\beta^{n})$} &
  \colhead{FWHM([O\,III])}     & \colhead{log$F(\rm [O\,III])$}   & \colhead{log$F(\rm Optical Fe\,II)$} &
  \colhead{log$M_{\rm BH}$} & \colhead{$L/L_{Edd}$} \\
  \colhead{}  &  \colhead{} &
  \colhead{erg~s$^{-1}$} & \colhead{km~s$^{-1}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$} &
  \colhead{ergs~s$^{-1}$~cm$^{-2}$} &
  \colhead{km~s$^{-1}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$} & \colhead{ergs~s$^{-1}$~cm$^{-2}$} &
  \colhead{$\msun$} & \colhead{}}
\startdata

 J010352.46+003739.7 & 0.705 & 44.97 & 4964 & -13.57 & -15.54 & -13.91 & 2913 & -13.66 & 8.63 & 0.15\\
 J014534.36+143136.9 & 0.636 & 44.27 & 7005 & -14.37 & -15.81 & -15.03 & 803  & -14.60 & 8.45 & 0.05\\
 J023102.49-083141.2 & 0.587 & 44.18 & 3812 & -14.23 & -16.36 & -14.78 & 1058 & -14.16 & 8.11 & 0.08\\
 J023153.64-093333.6 & 0.555 & 44.13 & 5557 & -14.27 & -16.08 & -15.23 & 707  & -14.50 & 8.27 & 0.05\\
 J024220.10-085332.7 & 0.800 & 44.43 & 5939 & -14.08 & -15.37 & -14.40 & 354  & -14.50 & 8.45 & 0.07\\
 J025026.66+000903.3 & 0.597 & 44.45 & 8448 & -14.28 & -16.15 & -14.53 & 521  & -14.58 & 8.62 & 0.05\\
 J033438.28-071149.0 & 0.635 & 44.92 & 4620 & -13.53 &        & -14.18 & 527  & -13.65 & 8.58 & 0.16\\
 J080248.19+551328.8 & 0.664 & 44.75 & 2264 & -14.09 & -14.98 & -14.34 & 782  & -13.84 & 8.15 & 0.28\\
 J080934.64+254837.9 & 0.545 & 44.54 & 8778 & -13.88 & -15.38 & -14.62 & 719  & -14.20 & 8.69 & 0.05\\
 J081655.34+074311.5 & 0.645 & 44.37 & 3964 & -14.19 & -16.07 & -14.56 & 992  & -14.23 & 8.23 & 0.10\\
 J082231.53+231152.0 & 0.653 & 44.86 & 9090 & -13.76 & -15.05 & -13.81 & 598  & -15.24 & 8.87 & 0.07\\
 J083000.35+343238.7 & 0.740 & 44.44 & 2030 & -14.52 &        & -15.24 & 241  &        & 7.94 & 0.22\\
 J083525.98+435211.3 & 0.568 & 44.77 & 2518 & -14.20 & -15.01 & -14.84 & 747  & -13.67 & 8.21 & 0.26\\
 J083613.23+280512.1 & 0.743 & 44.33 & 2004 & -14.37 &        & -15.25 & 388  & -14.54 & 7.88 & 0.20\\
 J084716.03+373218.0 & 0.453 & 44.62 & 2539 & -13.63 & -14.88 & -13.74 & 484  & -14.21 & 8.14 & 0.22\\
 J084824.14+034542.3 & 0.699 & 44.45 & 4179 & -13.95 & -15.38 & -14.02 & 522  & -15.08 & 8.29 & 0.10\\
 J085053.12+445122.4 & 0.542 & 44.72 & 8888 & -13.55 & -15.80 & -14.35 & 698  & -13.78 & 8.79 & 0.06\\
 J085215.65+492040.8 & 0.567 & 44.25 & 4917 & -14.28 & -15.66 & -15.01 & 360  & -14.40 & 8.27 & 0.07\\
 J085357.88+463350.6 & 0.549 & 44.53 & 4849 & -14.06 &        & -14.91 & 1453 & -13.98 & 8.40 & 0.10\\
 J091146.06+403501.0 & 0.441 & 44.12 & 1614 & -14.28 & -15.22 & -14.64 & 396  & -14.33 & 7.68 & 0.20\\
 J092035.59+524006.2 & 0.793 & 44.78 & 9735 & -14.01 & -15.53 & -14.56 & 874  & -14.79 & 8.86 & 0.06\\
 J092157.62+103539.0 & 0.548 & 44.05 & 1680 & -14.51 & -15.95 & -15.31 & 1126 & -14.34 & 7.66 & 0.18\\
 J092441.08-001729.6 & 0.707 & 44.84 & 4045 & -13.76 & -15.48 & -14.14 & 572  & -14.38 & 8.47 & 0.17\\
 J092928.63+324129.8 & 0.776 & 44.68 & 5212 & -14.05 & -15.63 & -14.72 & 1611 & -13.98 & 8.51 & 0.11\\
 J093034.79+570520.6 & 0.637 & 44.34 & 2072 & -14.55 & -15.39 & -15.21 & 874  & -14.25 & 7.90 & 0.19\\
 J093759.60+453801.8 & 0.429 & 44.08 & 13451& -13.81 & -15.26 & -13.97 & 578  & -14.06 & 8.66 & 0.02\\
 J094443.13+062507.4 & 0.695 & 45.46 & 5122 & -13.20 & -15.13 & -14.15 & 3107 & -13.36 & 8.89 & 0.26\\
 J094939.93+393642.9 & 0.654 & 43.95 & 1330 & -14.71 & -15.82 & -15.16 & 615  & -14.68 & 7.50 & 0.20\\
 J101151.95+542942.6 & 0.536 & 43.93 & 1640 & -14.35 & -15.13 & -14.02 & 412  & -15.33 & 7.59 & 0.16\\
 J101203.31+492148.2 & 0.748 & 44.57 & 5299 & -14.79 & -17.00 & -15.58 & 1087 & -14.56 & 8.47 & 0.09\\
 J102021.21+121909.1 & 0.480 & 44.23 & 2620 & -14.39 & -15.24 & -15.17 & 1114 & -14.16 & 7.96 & 0.13\\
 J102802.33+592906.7 & 0.536 & 43.93 & 4313 & -14.27 & -16.76 & -14.85 & 2186 & -14.30 & 8.05 & 0.05\\
 J102839.11+450009.4 & 0.585 & 45.03 & 4510 & -13.39 & -15.00 & -14.29 & 501  & -13.78 & 8.62 & 0.18\\
 J103824.47-010538.9 & 0.773 & 44.52 & 2088 & -14.61 & -15.80 & -14.46 & 377  & -16.34 & 8.00 & 0.24\\
 J104132.96+513657.0 & 0.735 & 44.70 & 5698 & -14.10 & -15.18 & -14.69 & 4650 & -13.92 & 8.56 & 0.10\\
 J104210.43+501609.1 & 0.789 & 44.89 & 5828 & -14.63 &        & -15.11 & 4186 & -14.99 & 8.67 & 0.12\\
 J104459.60+365605.1 & 0.701 & 45.20 & 4221 & -13.46 &        & -14.27 & 4608 & -13.44 & 8.67 & 0.24\\
 J104705.08+590728.4 & 0.392 & 44.26 & 8965 & -14.06 & -15.75 & -14.62 & 415  & -14.22 & 8.56 & 0.04\\
 J105102.78+525049.8 & 0.543 & 44.16 & 7029 & -14.13 &        & -15.01 & 436  & -14.59 & 8.40 & 0.04\\
 J105259.99+065358.0 & 0.724 & 44.48 & 2116 & -14.15 &        & -15.21 & 641  & -14.19 & 7.98 & 0.22\\
 J105404.72+042939.3 & 0.579 & 44.08 & 7923 & -14.25 & -15.84 & -14.30 & 562  & -14.63 & 8.41 & 0.03\\
 J112632.81+430938.5 & 0.436 & 44.39 & 3990 & -13.94 &        & -14.84 & 980  & -14.03 & 8.24 & 0.10\\
 J112730.71+423039.0 & 0.531 & 44.57 & 2664 & -13.96 & -15.6  & -14.31 & 396  & -14.57 & 8.14 & 0.19\\
 J112822.42+482310.1 & 0.541 & 44.79 & 4839 & -13.87 & -15.75 & -14.78 & 1892 & -13.83 & 8.53 & 0.13\\
 J112912.27+422853.9 & 0.582 & 44.28 & 1197 & -14.09 & -15.77 & -14.76 & 1802 & -14.15 & 7.61 & 0.33\\
 J113355.22+111208.8 & 0.763 & 44.42 & 4606 & -14.63 & -16.13 & -15.53 & 403  & -14.28 & 8.32 & 0.09\\
 J113807.83+531231.6 & 0.790 & 44.65 & 3993 & -14.46 & -15.91 & -14.83 & 388  & -14.49 & 8.37 & 0.14\\
 J114043.62+532438.9 & 0.530 & 44.31 & 6397 & -13.93 & -15.91 & -14.61 & 591  & -14.11 & 8.42 & 0.05\\
 J114209.01+070957.7 & 0.497 & 44.34 & 2154 & -14.47 & -15.40 & -15.10 & 524  & -14.11 & 7.92 & 0.19\\
 J114915.30+393325.4 & 0.630 & 44.19 & 1307 & -14.38 & -15.53 & -14.69 & 1376 & -14.46 & 7.61 & 0.27\\
 J115816.72+132624.1 & 0.440 & 44.59 & 1788 & -13.69 & -15.56 & -14.19 & 383  & -13.66 & 7.96 & 0.30\\
 J120146.46+630034.4 & 0.659 & 44.17 & 11015& -14.21 & -15.63 & -14.54 & 364  & -15.40 & 8.61 & 0.03\\
 J120924.07+103612.0 & 0.395 & 44.90 & 7764 & -12.93 & -14.45 & -13.22 & 581  & -14.00 & 8.81 & 0.09\\
 J120928.11+003511.6 & 0.610 & 43.99 & 2663 & -14.71 &        & -15.46 & 596  & -14.52 & 7.85 & 0.10\\
 J121113.38+121937.3 & 0.465 & 44.19 & 3946 & -13.73 & -15.49 & -14.44 & 1498 & -13.95 & 8.13 & 0.08\\
 J121303.40-014450.9 & 0.613 & 44.47 & 2928 & -14.04 & -15.43 & -14.72 & 989  & -14.14 & 8.13 & 0.16\\
 J121907.80-005609.2 & 0.638 & 44.00 & 3183 & -14.39 &        & -15.29 & 1416 & -14.27 & 7.94 & 0.08\\
 J122043.21-013215.3 & 0.448 & 43.87 & 10914& -14.16 & -15.00 & -14.01 & 602  & -14.90 & 8.46 & 0.02\\
 J122703.19+505356.2 & 0.765 & 44.85 & 4060 & -13.90 & -15.05 & -14.35 & 1238 & -14.35 & 8.48 & 0.17\\
 J124300.87+153510.6 & 0.562 & 44.40 & 6862 & -13.90 &        & -14.26 & 564  & -14.52 & 8.50 & 0.06\\
 J130741.12+503106.4 & 0.695 & 44.75 & 4863 & -14.14 & -16.83 & -15.31 & 1168 & -14.11 & 8.51 & 0.12\\
 J131823.73+123812.5 & 0.589 & 44.17 & 6768 & -14.48 & -16.33 & -15.33 & 1389 & -14.30 & 8.38 & 0.04\\
 J132114.42+020225.0 & 0.582 & 44.07 & 1548 & -14.29 &        & -14.84 & 2258 & -14.22 & 7.63 & 0.20\\
 J133936.69+111949.2 & 0.650 & 44.32 & 2076 & -14.28 & -15.35 & -15.06 & 1404 & -14.18 & 7.90 & 0.19\\
 J134127.40+002050.5 & 0.722 & 44.42 & 3780 & -14.16 &        & -14.74 & 1600 & -14.35 & 8.23 & 0.11\\
 J134415.75+331719.1 & 0.687 & 44.56 & 2028 & -13.97 & -15.91 & -13.91 & 1168 & -14.79 & 8.00 & 0.26\\
 J135418.26+585935.9 & 0.791 & 44.36 & 2512 & -14.23 & -15.6  & -14.69 & 468  & -14.33 & 8.01 & 0.16\\
 J140025.53-012957.0 & 0.584 & 44.50 & 3600 & -14.40 & -15.26 & -15.20 & 769  & -14.05 & 8.25 & 0.13\\
 J140115.74+621857.1 & 0.645 & 44.36 & 2691 & -14.31 & -16.13 & -15.11 & 430  & -14.30 & 8.04 & 0.15\\
 J142647.47+401250.8 & 0.749 & 44.39 & 13107& -13.91 & -15.65 & -14.49 & 582  & -14.74 & 8.80 & 0.03\\
 J142649.24+032517.7 & 0.529 & 44.36 & 5114 & -14.06 &        & -14.94 & 1714 & -14.18 & 8.34 & 0.07\\
 J142927.28+523849.5 & 0.595 & 44.84 & 3034 & -13.59 & -14.88 & -14.18 & 2880 & -13.63 & 8.34 & 0.23\\
 J143303.27+403105.1 & 0.446 & 44.03 & 3914 & -14.18 & -16.08 & -14.78 & 419  & -14.30 & 8.05 & 0.07\\
 J143828.63+452108.6 & 0.427 & 44.12 & 2355 & -14.01 &        & -14.68 & 1086 & -13.97 & 7.86 & 0.13\\
 J144342.21-025430.6 & 0.777 & 44.36 & 1571 & -14.22 &        & -15.11 & 1676 & -14.34 & 7.78 & 0.27\\
 J144642.26+454630.9 & 0.738 & 44.58 & 5527 & -14.39 &        &        &      & -14.24 & 8.49 & 0.09\\
 J144903.18+503018.1 & 0.609 & 44.22 & 1980 & -14.36 &        & -14.71 & 977  & -14.45 & 7.82 & 0.18\\
 J145724.00+452157.8 & 0.718 & 44.55 & 1889 & -14.18 &        & -15.11 & 1290 & -14.18 & 7.97 & 0.28\\
 J145736.70+523454.6 & 0.638 & 44.60 & 3024 & -14.30 & -15.39 & -14.72 & 1687 & -13.88 & 8.21 & 0.17\\
 J145836.73+433015.5 & 0.760 & 44.60 & 3706 & -14.22 &        & -14.98 & 1931 & -14.25 & 8.31 & 0.14\\
 J150847.41+340437.7 & 0.788 & 45.04 & 6361 & -13.10 & -14.66 & -13.37 & 713  & -14.43 & 8.79 & 0.13\\
 J151225.67+585752.2 & 0.791 & 44.45 & 12348& -14.64 &        &        &      & -14.15 & 8.80 & 0.03\\
 J151545.34+031745.0 & 0.780 & 44.29 & 14057& -14.06 & -15.99 & -14.75 & 1059 & -14.63 & 8.78 & 0.02\\
 J151548.67+430420.5 & 0.527 & 44.05 & 1554 & -14.33 & -15.74 & -14.75 & 382  & -14.36 & 7.62 & 0.19\\
 J153036.83+370439.2 & 0.417 & 44.42 & 1408 & -13.53 & -16.09 & -14.35 & 1258 & -13.72 & 7.76 & 0.33\\
 J160329.72+502722.2 & 0.638 & 44.28 & 4097 & -14.10 & -15.87 & -14.66 & 605  & -14.53 & 8.20 & 0.09\\
 J160628.06+290333.8 & 0.434 & 44.64 & 2232 & -13.75 &        & -14.41 & 1133 & -13.79 & 8.09 & 0.25\\
 J160721.27+515510.6 & 0.776 & 44.24 & 1544 & -14.44 & -16.03 & -15.23 & 926  & -14.34 & 7.71 & 0.24\\
 J161425.17+375210.7 & 0.553 & 44.93 & 5502 & -13.43 & -14.98 & -14.20 & 998  & -13.53 & 8.66 & 0.13\\
 J163255.46+420407.8 & 0.728 & 44.48 & 13320& -14.09 & -16.05 & -14.82 & 1243 & -14.52 & 8.85 & 0.03\\
 J163513.51+213859.6 & 0.683 & 44.25 & 1934 & -14.53 &        & -15.25 & 724  & -14.22 & 7.83 & 0.19\\
 J164447.19+311437.2 & 0.690 & 44.79 & 3996 & -13.87 & -16.07 & -14.51 & 337  & -13.86 & 8.44 & 0.16\\
 J165225.39+215830.7 & 0.447 & 44.56 & 2468 & -14.18 & -14.96 & -14.67 & 1109 & -14.11 & 8.10 & 0.21\\
 J170010.82+395545.8 & 0.577 & 44.19 & 1918 & -14.86 & -15.64 & -15.20 & 281  & -14.71 & 7.79 & 0.18\\
 J170330.23+324201.8 & 0.636 & 44.24 & 11088& -14.22 & -15.98 & -14.84 & 588  & -14.80 & 8.65 & 0.03\\
 J170341.82+383944.7 & 0.554 & 44.43 & 7083 & -14.02 & -15.91 & -14.57 & 396  & -14.31 & 8.53 & 0.06\\
 J204333.20-001104.2 & 0.544 & 44.61 & 2988 & -13.89 & -15.33 & -14.63 & 1092 & -13.86 & 8.21 & 0.18\\
 J210757.67-062010.6 & 0.644 & 45.03 & 11389& -13.42 & -14.97 & -14.00 & 1105 & -13.55 & 9.06 & 0.07\\
 J224028.14-003813.1 & 0.658 & 44.52 & 5876 & -14.16 & -16.28 & -15.00 & 255  & -14.43 & 8.49 & 0.08\\
{\it (This table is available in its entirety in a machine-readable form in the online
journal. A portion is shown here for guidance regarding its form and content.)}

\end{deluxetable}
\end{landscape}



